No-Regret Prediction in Marginally Stable Systems

We consider the problem of online prediction in a marginally stable linear dynamical system subject to bounded adversarial or (non-isotropic) stochastic perturbations. This poses two challenges. Firstly, the system is in general unidentifiable, so recent and classical results on parameter recovery do not apply. Secondly, because we allow the system to be marginally stable, the state can grow polynomially with time; this causes standard regret bounds in online convex optimization to be vacuous. In spite of these challenges, we show that the online least-squares algorithm achieves sublinear regret (improvable to polylogarithmic in the stochastic setting), with polynomial dependence on the system's parameters. This requires a refined regret analysis, including a structural lemma showing the current state of the system to be a small linear combination of past states, even if the state grows polynomially. By applying our techniques to learning an autoregressive filter, we also achieve logarithmic regret in the partially observed setting under Gaussian noise, with polynomial dependence on the memory of the associated Kalman filter.

==> format/defs_colt.tex <==
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{definition}{Definition}[section]
%\newtheorem{example}[theorem]{Example}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{application}[theorem]{Application}
%\newtheorem{optimizationproblem}[theorem]{Optimization~Problem}

\usepackage{algorithm}
\usepackage{algpseudocode}
\algnewcommand\algorithmicinput{\textbf{Input: }}
\algnewcommand\INPUT{\State\algorithmicinput}
\algnewcommand\algorithmicinitialize{\textbf{Initialize: }}
\algnewcommand\INIT{\State\algorithmicinitialize}
\algnewcommand\algorithmicrun{\textbf{Run: }}
\algnewcommand\RUN{\State\algorithmicrun}
\algnewcommand\algorithmicupdate{\textbf{Update: }}
\algnewcommand\UPDATE{\State\algorithmicupdate}
\algnewcommand\algorithmicset{\textbf{Set: }}
\algnewcommand\SET{\State\algorithmicset}
\algnewcommand\algorithmicquery{\textbf{Query: }}
\algnewcommand\QUERY{\State\algorithmicquery}
\algnewcommand\algorithmicoutput{\textbf{Output: }}
\algnewcommand\OUTPUT{\State\algorithmicoutput}

%\newcommand{\todo}[1]{\textbf{\textcolor{red}{TODO: #1}}}
\newcommand{\cz}[1]{\textbf{\textcolor{blue}{CZ: #1}}}
\newcommand{\hl}[1]{\textbf{\textcolor{purple}{HL: #1}}}
\newcommand{\yz}[1]{\textsf{\color{orange} YZ: #1}}
\newcommand{\ug}[1]{\textsf{\color{green} UG: #1}}
\newcommand{\ks}[1]{\textsf{\color{red} KS: #1}}

\DeclareMathOperator{\clip}{clip}
\def\norm#1{\mathopen\| #1 \mathclose\|}% use instead of $\|x\|$

\newcommand{\ellipsoid}{{\mathcal E}}
\newcommand{\sround}{\mathop{\mbox{\rm SmartRound}}}
\newcommand{\round}{\mathop{\mbox{\rm round}}}
\newcommand{\myspan}{\mathop{\mbox{\rm span}}}
\newcommand{\edges}{\mathop{\mbox{\rm edges}}}
\newcommand{\conv}{\mathop{\mbox{\rm conv}}}
\newcommand{\poly}{\mathop{\mbox{\rm poly}}}
\newcommand{\rank}{\mathop{\mbox{\rm rank}}}
\def\regret{\mbox{{Regret}}}
\DeclareMathOperator{\spn}{span}

\newcommand{\ignore}[1]{}
\newcommand{\equaldef}{\stackrel{\text{\tiny def}}{=}}
\newcommand{\equaltri}{\triangleq}
\newcommand{\tr}{\ensuremath{{\scriptscriptstyle\mathsf{T}}}}
\def\trace{{\bf Tr}}
\def\dist{{\bf P}}
\def\mydist{{\bf Q}}
\def\reals{{\mathbb R}}

%\newcommand\E{\mbox{\bf E}}
\newcommand\ball{\mathbb{B}}
\newcommand\var{\mbox{VAR}}
\newcommand\Lcal{\mathcal{L}}
\def\bzero{\mathbf{0}}

\def\Exp{\mathop{\mbox{E}}}
\def\mP{{\mathcal P}}
\def\risk{{\mbox{Risk}}}
\def\ent{{\mbox{ent}}}
\def\mG{{\mathcal G}}
\def\mA{{\mathcal A}}
\def\lhat{\hat{\ell}}
\def\Lhat{\hat{L}}
\def\ltil{\tilde{\ell}}
\def\Ltil{\tilde{L}}
\def\H{{\mathcal H}}

\def\Ahat{\hat{\mathbf{A}}}

\def\bold0{\mathbf{0}}
\def\boldone{\mathbf{1}}
\def\boldp{\mathbf{p}}
\def\boldq{\mathbf{q}}
\def\boldr{\mathbf{r}}
\def\boldA{\mathbf{A}}
\def\boldI{\mathbf{I}}
\newcommand\mycases[4] {{
\left\{
\begin{array}{ll}
    {#1} & {#2} \\\\
    {#3} & {#4}
\end{array}
\right. }}
\newcommand\mythreecases[6] {{
\left\{
\begin{array}{ll}
    {#1} & {#2} \\\\
    {#3} & {#4} \\\\
    {#5} & {#6}
\end{array}
\right. }}
\def\bb{\mathbf{b}}
%\def\bc{\mathbf{c}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
%\def\be{\mathbf{e}}
\def\etil{\tilde{\mathbf{e}}}
\def\bk{\mathbf{k}}
\def\bu{\mathbf{u}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}

\def\bw{\mathbf{w}}
%\def\ba{\mathbf{a}}
\def\bA{\mathbf{A}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bV{\mathbf{V}}
\def\bone{\mathbf{1}}


\def\xhat{\hat{\mathbf{x}}}
\def\xbar{\bar{\mathbf{x}}}
\def\vol{\mbox{vol}}
\def\trace{{\bf Tr}}
\def\Exp{\mathop{\mbox{E}}}
\newcommand{\val}{\mathop{\mbox{\rm val}}}
\renewcommand{\deg}{\mathop{\mbox{\rm deg}}}
%\newcommand{\eps}{\varepsilon}

% Macros for this chapter
\def\bone{\mathbf{1}}
\newcommand{\sphere}{\ensuremath{\mathbb {S}}}
\newcommand{\simplex}{\ensuremath{\Delta}}
\newcommand{\Ktil}{\ensuremath{\mathcal{\tilde{K}}}}
\def\mA{{\mathcal A}}
\newcommand{\rv}[1][t]{\ensuremath{\mathbf r_{#1}}}
\newcommand{\z}{\ensuremath{\mathbf z}}
\newcommand{\xtil}[1][t]{\ensuremath{\mathbf {\tilde{x}}_{#1}}}
\newcommand{\xv}[1][t]{\ensuremath{\mathbf x_{#1}}}
\newcommand{\xvh}[1][t]{\ensuremath{\mathbf {\hat x}}_{#1}}
\newcommand{\ftildeh}[1][t]{\ensuremath{\mathbf {\hat f}}_{#1}}
\newcommand{\xvbar}[1][t]{\ensuremath{\bar{\mathbf x}_{#1}}}
\newcommand{\xstar}{\ensuremath{\mathbf x^{*}}}
\newcommand{\xstarr}{\ensuremath{\mathbf x^{\star}}}
\newcommand{\yv}[1][t]{\ensuremath{\mathbf y_{#1}}}
\newcommand{\zv}[1][t]{\ensuremath{\mathbf z_{#1}}}
\newcommand{\fv}[1][t]{\ensuremath{\mathbf f_{#1}}}
\newcommand{\gv}[1][t]{\ensuremath{\mathbf g_{#1}}}
\newcommand{\qv}[1][t]{\ensuremath{\mathbf q_{#1}}}
\newcommand{\pv}[1][t]{\ensuremath{\mathbf p_{#1}}}
\newcommand{\ftilde}[1][t]{\ensuremath{\mathbf {\tilde f}_{#1}}}
\newcommand{\gtilde}[1][t]{\ensuremath{\mathbf {\tilde g}_{#1}}}
\newcommand{\lowtrace}{\mathcal{T}}

\newcommand{\ev}[1][i]{\ensuremath{\mathbf e_{#1}}}
\newcommand{\uv}{\ensuremath{\mathbf u}}
\newcommand{\ww}{\ensuremath{\mathbf w}}
\newcommand{\vv}{\ensuremath{\mathbf v}}
\newcommand{\A}[1][t]{\ensuremath{\mathbf A_{#1}}}
\newcommand{\Ftilde}[1][t]{\ensuremath{\mathbf {\tilde F}_{#1}}}
\newcommand{\Gtilde}[1][t]{\ensuremath{\mathbf {\tilde G}_{#1}}}
\newcommand{\hessum}[1][t]{\ensuremath{\boldsymbol{H}_{1:#1}}}
\newcommand{\reg}[1][t]{\ensuremath{\lambda_{#1}}}
\newcommand{\regsum}[1][t]{\ensuremath{\boldsymbol{\lambda}_{1:#1}}}
\newcommand{\bM}{\ensuremath{\mathcal M}}
%\newcommand{\F}{\ensuremath{\mathcal F}}
\newcommand{\ntil}{\tilde{\nabla}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\rhotil}{\tilde{\rho}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\mutil}{\tilde{\mu}}
\newcommand{\Atil}{\tilde{A}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\vtil}{\tilde{v}}
\newcommand\super[1] {{^{(#1)}}}
%\newcommand\pr{\mbox{\bf Pr}}
\newcommand\av{\mbox{\bf E}}
\def\bb{\mathbf{b}}
%\def\bB{\mathbf{B}}
\def\bB{{B}}
%\def\bC{\mathbf{C}}
\def\bC{{C}}
\def\bS{\mathbf{S}}
%\def\be{\mathbf{e}}
\def\bu{\mathbf{u}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bp{\mathbf{p}}
\def\bdelta{\mathbf{\delta}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bv{\mathbf{v}}
%\def\ba{\mathbf{a}}
%\def\bA{\mathbf{A}}
\def\bA{{A}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bP{\mathbf{P}}
\def\bV{\mathbf{V}}
\def\sgn{\text{sgn}}
\def\eps{\varepsilon}
\def\epsilon{\varepsilon}
\def\tsum{{\textstyle \sum}}
\def\universal{{\sc Universal}\xspace}
\def\ogd{{\sc Online Gradient Descent}\xspace}


% modifiers
%\newcommand{\obar}[1]{\overline{#1}}
\newcommand{\ubar}[1]{\underline{#1}}
\newcommand{\defeq}{\stackrel{\text{def}}{=}}

% brackets
\newcommand{\braces}[1]{\left\{#1\right\}}
%\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\ang}[1]{\left<#1\right>}
\newcommand{\bra}[1]{\left[#1\right]}
\newcommand{\abs}[1]{\left|#1\right|}

% matrices, fractions, derivatives
\newcommand{\mat}[1]{\begin{matrix}#1\end{matrix}}
\newcommand{\pmat}[1]{\pa{\mat{#1}}}
\newcommand{\bmat}[1]{\bra{\mat{#1}}}
\newcommand{\sismat}[1]{\left\{\mat{#1}\right.}
\newcommand{\sm}[1]{\begin{smallmatrix}#1\end{smallmatrix}}
\newcommand{\psm}[1]{\pa{\sm{#1}}}
\newcommand{\bsm}[1]{\bra{\sm{#1}}}
\newcommand{\tci}[2]{\set{\,#1 \mid{} #2\,}}
\newcommand{\tcia}[2]{\ang{\,#1 \mid{} #2\,}}
\newcommand{\pfrac}[2]{\pa{\frac{#1}{#2}}}
\newcommand{\bfrac}[2]{\bra{\frac{#1}{#2}}}
\newcommand{\psfrac}[2]{\pa{\sfrac{#1}{#2}}}
\newcommand{\bsfrac}[2]{\bra{\sfrac{#1}{#2}}}
\newcommand{\der}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pder}[2]{\pfrac{\partial #1}{\partial #2}}
\newcommand{\sder}[2]{\sfrac{\partial #1}{\partial #2}}
\newcommand{\psder}[2]{\psfrac{\partial #1}{\partial #2}}
\newcommand{\case}[1]{\begin{cases}#1\end{cases}}

% operators
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator{\Var}{\operatorname{Var}}
\DeclareMathOperator{\Cov}{\operatorname{Cov}}

% letters
\newcommand{\CC}{\mathbb{C}}
%\newcommand{\eps}{\varepsilon}


% theorems
%\newtheorem{theorem}{theorem}[section]
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{asm}[theorem]{Assumption}
\newtheorem{cor}[theorem]{Corollary}
%\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{df}[theorem]{Definition}
%\newtheorem*{df*}[theorem]{Definition}
%\newtheorem{definition}[theorem]{Definition}
\newtheorem{lem}[theorem]{Lemma}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{remark}[theorem]{Remark}
\newtheorem{rem}[theorem]{Remark}
\newtheorem*{rem*}{Remark}
\newtheorem{pr}[theorem]{Proposition}
\newtheorem*{pr*}{Proposition}
% environment shorthands
\newcommand{\eqn}[1]{\begin{equation}#1\end{equation}}



%\theoremstyle{definition}

\DeclareMathOperator*\E{\mathbb{E}}
\newcommand\R{\mathbb{R}}
\newcommand\Sph{\mathbb{S}}
\newcommand\C{\mathbb{C}}
\newcommand\w{\mathbf{w}}
\newcommand\bias{\mathbf{b}}
\newcommand\ome{\mathbf{\omega}}
\newcommand\Y{\mathbf{Y}}
\newcommand\K{\mathbf{K}}
%\newcommand\N{\mathcal{N}}
\newcommand\D{\mathcal{D}}
\newcommand\U{\mathcal{U}}
\newcommand\V{\mathcal{V}}
\newcommand\X{\mathcal{X}}
\newcommand\sig{\mathcal{\sigma}}
\newcommand\x{\mathbf{x}}
\newcommand\y{\mathbf{y}}
%\newcommand\al{\boldsymbol{\alpha}}

\def\Pbb{\mathbb{P}}

\renewcommand\t{{\scriptscriptstyle\top}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Astar}{\tilde{A}}
\DeclareMathOperator{\Bstar}{\tilde{B}}
\DeclareMathOperator{\Cstar}{\tilde{C}}
\DeclareMathOperator{\wstar}{\tilde{w}}
\DeclareMathOperator{\astar}{\tilde{a}}
\DeclareMathOperator{\bstar}{\tilde{b}}
\DeclareMathOperator{\cstar}{\tilde{c}}
\newcommand\wh{\widehat}
\newcommand\wt{\widetilde}
%\newcommand\eps{\varepsilon}
%\newcommand\veps{\varepsilon}
\newcommand\h{\hat}

\DeclareMathOperator{\MMD}{\mathrm{MMD}}

\newcommand\tl{\tilde}
%\newcommand\bar{\overline}
\newcommand\inner[1]{\langle #1 \rangle}
\newcommand\sign{\operatorname{sign}}
\newcommand{\Ds}{\mathcal{D}_{synth}}
\newcommand{\Dr}{\mathcal{D}_{real}}
\newcommand\indicator[1]{\ensuremath{\mathbf{1}_{#1}}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}

\newcommand{\grad}{\nabla}
\newcommand{\G}{\mathbf{G}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bSig}{\mathbf{\Sigma}}

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cH}{\mathcal{H}}

%authornote
\def\shownotes{1}  \ifnum\shownotes=1
\newcommand{\authnote}[2]{$\ll$\textsf{\footnotesize #1 notes: #2}$\gg$}
\else
\newcommand{\authnote}[2]{}
\fi
\newcommand{\hlnote}[1]{{\color{purple}\authnote{HL}{#1}}}

\newcommand{\st}[0]{\mathscr{st}}

%LETTERS

%UPPERCASE
\newcommand{\KL}[0]{\operatorname{KL}}
\newcommand{\sA}[0]{\mathscr{A}}
\newcommand{\cA}[0]{\mathcal{A}}
%\newcommand{\A}[0]{\mathbb{A}}
\newcommand{\cB}[0]{\mathcal{B}}
%\newcommand{\C}[0]{\mathbb{C}}
\newcommand{\sC}[0]{\mathcal{C}}%deprecated
\newcommand{\cC}[0]{\mathcal{C}}
\newcommand{\sD}[0]{\mathscr{D}}
\newcommand{\mD}[0]{\mathfrak D}
\newcommand{\cE}[0]{\mathscr{E}}%deprecated
\newcommand{\sE}[0]{\mathscr{E}}
%\newcommand{\E}[0]{\mathbb{E}}
\newcommand{\EE}[0]{\mathop{\mathbb E}}
%\scalebox{1.25}{$\mathbb E$}}
\newcommand{\F}[0]{\mathbb{F}}
\newcommand{\cF}[0]{\mathcal{F}}%deprecated.
\newcommand{\sF}[0]{\mathscr{F}}
%\newcommand{\G}[0]{\mathbb{G}}
\newcommand{\cG}[0]{\mathscr{G}}%deprecated.
\newcommand{\sG}[0]{\mathscr{G}}
%\newcommand{\cH}[0]{\mathcal H}%deprecated
\newcommand{\sH}[0]{\mathscr H}
\newcommand{\Hq}[0]{\mathbb{H}}
\newcommand{\bfI}[0]{\mathbf{I}}
\newcommand{\I}[0]{\mathbb{I}}
\newcommand{\cI}[0]{\mathscr{I}}%deprecated
\newcommand{\sI}[0]{\mathscr{I}}
\newcommand{\cJ}[0]{\mathscr{J}}
\newcommand{\cL}[0]{\mathscr{L}}
\newcommand{\N}[0]{\mathbb{N}}
\newcommand{\fN}[0]{\mathfrak{N}}
\newcommand{\cP}[0]{\mathcal{P}}
\newcommand{\Pj}[0]{\mathbb{P}}
%\newcommand{\mP}[0]{\mathfrak{P}}
\newcommand{\mQ}[0]{\mathfrak{Q}}
%!
\newcommand{\cO}[0]{\mathcal{O}}
\newcommand{\sO}[0]{\mathscr{O}}
\newcommand{\Q}[0]{\mathbb{Q}}
%\newcommand{\R}[0]{\mathbb{R}}
%\newcommand{\bS}[0]{\mathbb{S}}
\newcommand{\T}[0]{\mathbb{T}}
%\newcommand{\X}[0]{\mathfrak{X}}
\newcommand{\Z}[0]{\mathbb{Z}}
\newcommand{\one}[0]{\mathbbm{1}}
%lowercase
\newcommand{\mba}[0]{\mathbf{a}}%idele a
\newcommand{\ma}[0]{\mathfrak{a}}%ideal a
\newcommand{\mb}[0]{\mathfrak{b}}
\newcommand{\mc}[0]{\mathfrak{c}}
\newcommand{\mfd}[0]{\mathfrak d}
\newcommand{\mf}[0]{\mathfrak{f}}
\newcommand{\fg}[0]{\mathfrak{g}}
\newcommand{\vi}[0]{\mathbf{i}}%vector i
\newcommand{\vj}[0]{\mathbf{j}}
\newcommand{\vk}[0]{\mathbf{k}}
\newcommand{\mm}[0]{\mathfrak{m}}%ideal m
\newcommand{\mfp}[0]{\mathfrak{p}}
\newcommand{\mq}[0]{\mathfrak{q}}
\newcommand{\mr}[0]{\mathfrak{r}}
\newcommand{\mv}[0]{\mathbf{v}}
\newcommand{\mx}[0]{\mathbf{x}}%idele x
\newcommand{\my}[0]{\mathbf{y}}
%More sequences of letters
\newcommand{\et}[0]{_{\text{\'et}}}
\newcommand{\Gm}[0]{\mathbb{G}_m}
\newcommand{\Fp}[0]{\mathbb{F}_p}
\newcommand{\fq}[0]{\mathbb{F}_q}
\newcommand{\fpb}[0]{\ol{\mathbb{F}_p}}
\newcommand{\fpt}[0]{\mathbb{F}_p^{\times}}
\newcommand{\fqt}[0]{\mathbb{F}_q^{\times}}
\newcommand{\Kt}[0]{K^{\times}}
\newcommand{\RP}[0]{\mathbb{R}P}
\newcommand{\qb}[0]{\ol{\mathbb{Q}}}
\newcommand{\qp}[0]{\mathbb{Q}_p}
\newcommand{\qpb}[0]{\ol{\mathbb{Q}_p}}
\newcommand{\ql}[0]{\mathbb Q_{\ell}}
\newcommand{\sll}[0]{\mathfrak{sl}}
\newcommand{\vl}[0]{V_{\ell}}
\newcommand{\zl}[0]{\mathbb Z_{\ell}}
\newcommand{\zp}[0]{\mathbb Z_{p}}
\newcommand{\zpz}[0]{\mathbb Z/p\mathbb Z}
%Shortcuts for greek letters
\newcommand{\al}[0]{\alpha}
\newcommand{\be}[0]{\beta}
\newcommand{\ga}[0]{\gamma}
\newcommand{\Ga}[0]{\Gamma}
\newcommand{\de}[0]{\delta}
\newcommand{\De}[0]{\Delta}
\newcommand{\ep}[0]{\varepsilon}
\newcommand{\eph}[0]{\frac{\varepsilon}{2}}
\newcommand{\ept}[0]{\frac{\varepsilon}{3}}
\newcommand{\ka}[0]{\kappa}
\newcommand{\la}[0]{\lambda}
\newcommand{\La}[0]{\Lambda}
\newcommand{\ph}[0]{\varphi}
\newcommand{\Ph}[0]{\Phi}
\newcommand{\rh}[0]{\rho}
\newcommand{\te}[0]{\theta}
\newcommand{\Te}[0]{\Theta}
\newcommand{\vte}[0]{\vartheta}
\newcommand{\om}[0]{\omega}
\newcommand{\Om}[0]{\Omega}
\newcommand{\si}[0]{\sigma}
\newcommand{\Si}[0]{\Sigma}
\newcommand{\ze}[0]{\zeta}

%SYMBOLS

%Shortcuts for symbols
\newcommand{\nin}[0]{\not\in}
\newcommand{\opl}[0]{\oplus}
\newcommand{\bigopl}[0]{\bigoplus}
\newcommand{\ot}[0]{\otimes}
\newcommand{\bigot}[0]{\bigotimes}
\newcommand{\sub}[0]{\subset}
\newcommand{\nsub}[0]{\not\subset}
\newcommand{\subeq}[0]{\subseteq}
\newcommand{\supeq}[0]{\supseteq}
\newcommand{\nsubeq}[0]{\not\subseteq}
\newcommand{\nsupeq}[0]{\not\supseteq}
\newcommand{\nequiv}[0]{\not\equiv}
\newcommand{\bs}[0]{\backslash}
\newcommand{\iy}[0]{\infty}
\newcommand{\no}[0]{\trianglelefteq}%normal subgroup
\newcommand{\qeq}[0]{\stackrel?=}
\newcommand{\subsim}[0]{\stackrel{\sub}{\sim}}
\newcommand{\supsim}[0]{\stackrel{\supset}{\sim}}
\newcommand{\na}[0]{\nabla}
\newcommand{\mcv}[0]{*_-}
\newcommand{\dlim}[0]{\varinjlim}
\newcommand{\ilim}[0]{\varprojlim}
\newcommand{\gle}[0]{\begin{array}{c}
\ge\\
\le
\end{array}}
\newcommand{\lge}[0]{\begin{array}{c}
\le\\
\ge
\end{array}}
%\stackrel{-}{*}}%minus convoluion.

%COMMON TIME-SAVERS

%Fractions
\newcommand{\rc}[1]{\frac{1}{#1}}
\newcommand{\prc}[1]{\pa{\rc{#1}}}
\newcommand{\ff}[2]{\left\lfloor\frac{#1}{#2}\right\rfloor}
\newcommand{\cf}[2]{\left\lceil\frac{#1}{#2}\rceil\rfloor}
\newcommand{\fc}[2]{\frac{#1}{#2}}
\newcommand{\sfc}[2]{\sqrt{\frac{#1}{#2}}}
\newcommand{\pf}[2]{\pa{\frac{#1}{#2}}}%Shortcut for fraction with parentheses
\DeclareRobustCommand{\stl}{\genfrac\{\}{0pt}{}}

\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}%Partial derivatives
\newcommand{\dd}[2]{\frac{d #1}{d #2}}
\newcommand{\pdd}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ddd}[1]{\frac{d}{d #1}}
\newcommand{\af}[2]{\ab{\fc{#1}{#2}}}
\newcommand{\ddt}[2]{\frac{d^2 #1}{d {#2}^2}}
\newcommand{\pdt}[2]{\frac{\partial^2 #1}{\partial {#2}^2}}
\newcommand{\pdxy}[3]{\frac{\partial^2 #1}{\partial {#2}\partial {#3}}}
\newcommand{\pl}[0]{\partial}
\newcommand{\nb}[0]{\nabla}
\newcommand{\onb}[0]{\ol{\nabla}}
\newcommand{\dy}{\,dy}
\newcommand{\dx}{\,dx}

%Arrows
\newcommand{\lar}[0]{\leftarrow}
\newcommand{\ra}[0]{\rightarrow}
\newcommand{\dra}[0]{\dashrightarrow}
\newcommand{\lra}[0]{\leftrightarrow}
\newcommand{\rra}[0]{\twoheadrightarrow}
\newcommand{\hra}[0]{\hookrightarrow}
\newcommand{\tra}[0]{\twoheadrightarrow}
\newcommand{\send}[0]{\mapsto}
\newcommand{\xra}[1]{\xrightarrow{#1}}
\newcommand{\xla}[1]{\xleftarrow{#1}}
\newcommand{\xhra}[1]{\xhookrightarrow{#1}}
\newcommand{\xlra}[1]{\xleftrightarrow{#1}}
\newcommand{\xrc}[0]{\xrightarrow{\cong}}
%\renewcommand{\cir}[0]{\circlearrowright}
\newcommand{\cil}[0]{\circlearrowleft}

%Brackets
\newcommand{\ab}[1]{\left| {#1} \right|}
\newcommand{\an}[1]{\left\langle {#1}\right\rangle}
\newcommand{\ba}[1]{\left[ {#1} \right]}
\newcommand{\bc}[1]{\left\{ {#1} \right\}}
%\newcommand{\bra}[1]{\langle{#1}|}
\newcommand{\braa}[1]{\langle\langle{#1}|}
\newcommand{\ce}[1]{\left\lceil {#1}\right\rceil}
\newcommand{\fl}[1]{\left\lfloor {#1}\right\rfloor}
\newcommand{\ro}[1]{\left\lfloor {#1}\right\rceil}
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\kett}[1]{|{#1}\rangle\rangle}
%\newcommand{\bk}[2]{\langle{#1}|{#2}\rangle}
\newcommand{\braak}[2]{\langle\langle{#1}|{#2}\rangle\rangle}
\newcommand{\kbb}[1]{|{#1}\rangle\langle{#1}|}
\newcommand{\kb}[2]{|{#1}\rangle\langle{#2}|}
\newcommand{\kettb}[2]{|{#1}\rangle\rangle\langle\langle{#2}|}
\newcommand{\pa}[1]{\left( {#1} \right)}
\newcommand{\pat}[1]{\left( \text{#1} \right)}
\newcommand{\ve}[1]{\left\Vert {#1}\right\Vert}
\newcommand{\nv}[1]{\frac{#1}{\left\Vert {#1}\right\Vert}}
\newcommand{\nvl}[2]{\frac{#1}{\left\Vert {#1}\right\Vert_{#2}}}
\newcommand{\rb}[1]{\left.{#1}\right|}
%\newcommand{\nl}[1]{\left\Vert #1 \right\Vert_{L^1}}
\newcommand{\ad}[0]{|\cdot|}
\newcommand{\ved}[0]{\ve{\cdot}}
\renewcommand{\set}[2]{\left\{{#1}:{#2}\right\}}
\newcommand{\sett}[2]{\left\{\left.{#1}\right|{#2}\right\}}

%under and overlines, etc.
\newcommand{\ch}[1]{\check{#1}}
\newcommand{\dch}[1]{\check{\check{#1}}}
\newcommand{\olra}[1]{\overleftrightarrow{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ub}[2]{\underbrace{#1}_{#2}}
\newcommand{\ora}[1]{\overrightarrow{#1}}
\newcommand{\ura}[1]{\underrightarrow{#1}}
%\newcommand{\wt}[1]{\widetilde{#1}}
%\newcommand{\wh}[1]{\widehat{#1}}

%other
\newcommand{\fp}[1]{^{\underline{#1}}}%Falling power
\newcommand{\rp}[1]{^{\overline{#1}}}
\newcommand{\pp}[1]{^{(#1)}}
\newcommand{\sh}[0]{^{\sharp}}
\newcommand{\ri}[0]{\ddagger}%replace this with rosati involution
\newcommand{\bit}[0]{\{0,1\}}

%TEXT
\newcommand{\btih}[1]{\text{ by the induction hypothesis{#1}}}
\newcommand{\bwoc}[0]{by way of contradiction}
%\newcommand{\by}[1]{\text{by~(\ref{#1})}}
\newcommand{\idk}[0]{{\color{red}I don't know.} }
\newcommand{\ore}[0]{\text{ or }}
\newcommand{\wog}[0]{ without loss of generality }
\newcommand{\Wog}[0]{ Without loss of generality }
\newcommand{\step}[1]{\noindent{\underline{Step {#1}:}}}
\newcommand{\prt}[1]{\noindent{\underline{Part {#1}:}}}
\newcommand{\tfae}[0]{ the following are equivalent}
\newcommand{\fabfm}[0]{for all but finitely many }

%FUNCTIONS
%Functions, etc.
\newcommand{\Abs}{(\text{Ab}/S)}
\newcommand{\abk}{(\text{Ab}/k)}
\newcommand{\abc}{(\text{Ab}/\C)}
\newcommand{\Alb}{\operatorname{Alb}}
\newcommand{\Ann}{\operatorname{Ann}}
\newcommand{\Area}{\operatorname{Area}}
\newcommand{\amax}{\operatorname{argmax}}
\newcommand{\amin}{\operatorname{argmin}}
\newcommand{\Ass}{\operatorname{Ass}}
\newcommand{\Art}{\operatorname{Art}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\avg}{\operatorname{avg}}
%\newcommand{\bias}[0]{\operatorname{bias}}
\newcommand{\Binom}{\operatorname{Binom}}
\newcommand{\Bl}[0]{\operatorname{Bl}}
\newcommand{\Br}{\operatorname{Br}}
\newcommand{\chr}{\operatorname{char}}
\newcommand{\cis}{\operatorname{cis}}
\newcommand{\cl}{\operatorname{Cl}}
%\newcommand{\Cl}{C}%changed notation%this is confusing
\newcommand{\Cl}{\operatorname{Cl}}
\newcommand{\Coh}{\operatorname{Coh}}
\newcommand{\Coinf}[0]{\operatorname{Coinf}}
\newcommand{\Coind}[0]{\operatorname{Coind}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\colim}{\operatorname{colim}}
\newcommand{\Comp}{\operatorname{Comp}}
%\newcommand{\conv}{\operatorname{conv}}
\newcommand{\oconv}{\ol{\conv}}
\newcommand{\Cor}{\operatorname{Cor}}
%\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\cro}{\operatorname{cr}}
\newcommand{\degs}[0]{\deg_{\text{s}}}%separable degree
\newcommand{\Dec}{\operatorname{Dec}}
\newcommand{\depth}{\operatorname{depth}}
\newcommand{\Der}{\operatorname{Der}}
%\newcommand{\diag}{\operatorname{diag}}
\newcommand{\diam}{\operatorname{diam}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\Dir}{\operatorname{Dir}}
\newcommand{\Div}{\operatorname{Div}}
\newcommand{\Disc}{\operatorname{Disc}}%discrepancy
\newcommand{\disc}{\operatorname{disc}}%discriminant
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\Ell}{\mathcal{E}{\rm{ll}}}
\newcommand{\Enc}{\operatorname{Enc}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Ent}{\operatorname{Ent}}
\newcommand{\Ext}{\operatorname{Ext}}
%\newcommand{\Exp}{\operatorname{Exp}}
\newcommand{\err}{\operatorname{err}}
\newcommand{\ess}{\operatorname{ess}}
\newcommand{\ext}{\operatorname{ext}}
\newcommand{\pfcg}{(p\text{-FCGp}/k)}
\newcommand{\fcg}{(\text{FCGp}/k)}
\newcommand{\Frac}{\operatorname{Frac}}
\newcommand{\Frob}{\operatorname{Frob}}
\newcommand{\Fun}{\operatorname{Fun}}
\newcommand{\FS}{\operatorname{FS}}
\newcommand{\Gal}{\operatorname{Gal}}
\newcommand{\Gap}{\operatorname{Gap}}
%\newcommand{\grad}{\operatorname{grad}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\gps}{(\text{Gp}/S)}
\newcommand{\Hess}{\operatorname{Hess}}
\newcommand{\Het}{H_{\text{\'et}}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Homeo}{\operatorname{Homeo}}
\newcommand{\chom}[0]{\mathscr{H}om}
\newcommand{\Homc}{\operatorname{Hom}_{\text{cont}}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\im}[0]{\text{im}}
\newcommand{\imp}[0]{\im^{\text{pre}}}
\newcommand{\Ind}[0]{\operatorname{Ind}}
\newcommand{\Inf}[0]{\operatorname{Inf}}
\newcommand{\inv}[0]{\operatorname{inv}}
\newcommand{\Isoc}[0]{\operatorname{Isoc}}
\newcommand{\Isog}[0]{\operatorname{Isog}}
\newcommand{\Isom}[0]{\operatorname{Isom}}
\newcommand{\Jac}[0]{\operatorname{Jac}}
\newcommand{\li}[0]{\operatorname{li}}
\newcommand{\Li}[0]{\operatorname{li}}
\newcommand{\Lie}[0]{\operatorname{Lie}}
\newcommand{\Line}[0]{\operatorname{Line}}
\newcommand{\Lip}[0]{\operatorname{Lip}}
\newcommand{\lcm}[0]{\operatorname{lcm}}
\newcommand{\Mat}{\operatorname{Mat}}
\newcommand{\Mod}{\operatorname{Mod}}
\newcommand{\Dmod}{\Mod_{W[F,V]}^{\text{fl}}}
\newcommand{\nil}[0]{\operatorname{nil}}
\newcommand{\nm}{\operatorname{Nm}}
\newcommand{\NS}{\operatorname{NS}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\PDer}{\operatorname{PDer}}
\newcommand{\PGL}{\operatorname{PGL}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Pico}{\operatorname{Pic}^{\circ}}
\newcommand{\Pois}{\operatorname{Pois}}
%\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\PSL}{\operatorname{PSL}}
\newcommand{\Per}{\operatorname{Per}}
\newcommand{\perm}{\operatorname{perm}}
\newcommand{\PrePer}{\operatorname{PrePer}}
\newcommand{\Prob}{\operatorname{Prob}}
\newcommand{\Proj}{\operatorname{Proj}}
\newcommand{\Prj}[0]{\textbf{Proj}}
\newcommand{\QCoh}{\operatorname{QCoh}}
\newcommand{\Rad}{\operatorname{Rad}}
\newcommand{\range}{\operatorname{range}}
%\newcommand{\rank}{\operatorname{rank}}
\newcommand{\red}{\operatorname{red}}
\newcommand{\Reg}{\operatorname{Reg}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\Ric}{\operatorname{Ric}} %Ricci curvature
\newcommand{\rot}{\operatorname{rot}}
\newcommand{\Scal}{\operatorname{Scal}} %Ricci curvature
\newcommand{\schs}{(\text{Sch}/S)}
\newcommand{\schk}{(\text{Sch}/k)}
\newcommand{\se}{\text{se}}
\newcommand{\srank}{\text{srank}}
\newcommand{\hse}{\wh{\text{se}}}
\newcommand{\Sel}{\operatorname{Sel}}
\newcommand{\sens}{\operatorname{sens}}
\newcommand{\Set}{(\text{Set})}
%\newcommand{\sgn}{\operatorname{sign}}
%\newcommand{\sign}{\operatorname{sign}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\Specf}[2]{\Spec\pa{\frac{k[{#1}]}{#2}}}
\newcommand{\rspec}{\ul{\operatorname{Spec}}}
\newcommand{\Spl}{\operatorname{Spl}}
\newcommand{\spp}{\operatorname{sp}}
%\newcommand{\spn}{\operatorname{span}}
\newcommand{\Stab}{\operatorname{Stab}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\ssupp}{\operatorname{sing}\operatorname{supp}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\Th}{\operatorname{Th}}
\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\tor}{\operatorname{tor}}
\newcommand{\Tr}[0]{\operatorname{Tr}}
%\newcommand{\tr}[0]{\operatorname{tr}}
%\newcommand{\val}[0]{\text{val}}
%\newcommand{\Var}[0]{\operatorname{Var}}
%\newcommand{\var}[0]{\text{var}}
\newcommand{\vcong}{\operatorname{vcong}}
\newcommand{\Vol}[0]{\operatorname{Vol}}
%\newcommand{\vol}[0]{\text{vol}}
\providecommand{\cal}[1]{\mathcal{#1}}
\renewcommand{\cal}[1]{\mathcal{#1}}
\providecommand{\bb}[1]{\mathbb{#1}}
\renewcommand{\bb}[1]{\mathbb{#1}}

%Text super/subscripts
\newcommand{\abe}[0]{^{\text{ab}}}
\newcommand{\gal}[0]{^{\text{gal}}}%galois closure
\newcommand{\op}{^{\text{op}}}
\newcommand{\pre}[0]{^{\text{pre}}}
\newcommand{\rd}[0]{_{\text{red}}}
\newcommand{\sep}[0]{^{\text{sep}}}
\newcommand{\tp}{^{\text{top}}}
\newcommand{\tors}{_{\text{tors}}}
\newcommand{\ur}[0]{^{\text{ur}}}
\newcommand{\urt}[0]{^{\text{ur}\times}}

%COMMUTATIVE DIAGRAMS

%Commutative diagram shortcuts
\newcommand{\commsq}[8]{\xymatrix{#1\ar[r]^-{#6}\ar[d]_{#5} &#2\ar[d]^{#7} \\ #3 \ar[r]^-{#8} & #4}}
%Makes a diagram like this
%1->2
%|    |
%3->4
%Arguments 5, 6, 7, 8 on arrows
%  6
%5  7
%  8
\newcommand{\pull}[9]{
#1\ar@/_/[ddr]_{#2} \ar@{.>}[rd]^{#3} \ar@/^/[rrd]^{#4} & &\\
& #5\ar[r]^{#6}\ar[d]^{#8} &#7\ar[d]^{#9} \\}
\newcommand{\back}[3]{& #1 \ar[r]^{#2} & #3}
%Syntax:\pull 123456789 \back ABC
%1=upper left-hand corner
%2,3,4=arrows from upper LH corner, going down, diagonal, right
%5,6,7=top row (6 on arrow)
%8,9=middle rows (on arrows)
%A,B,C=bottom row
%composition
\newcommand{\cmp}[9]{
\xymatrix{
#1 \ar[r]^{#4}{#5} \ar@/_2pc/[rr]^{#8}_{#9} & #2 \ar[r]^{#6}_{#7} & #3
}
}
\newcommand{\ctr}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5}\ar[rd]^{#6}_{#7} && #2\ar[ld]_{#8}^{#9}\\
& #3 &
}
}
\newcommand{\ctrr}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5} && #2\\
& #3 \ar[lu]_{#6}^{#7}\ar[ru]_{#8}^{#9}&
}
}

\newcommand{\ctri}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5}\ar[rd]^{#6}_{#7} && #2\\
& #3 \ar[ru]^{#8}_{#9}&
}
}
\newcommand{\rcommsq}[8]{\xymatrix{#1 &#2\ar[l]_-{#6} \\ #3 \ar[u]^{#5} & #4 \ar[u]_{#7}\ar[l]_-{#8}}}


%Arrow shortcuts
\newcommand{\ha}[1]{\ar@{^(->}[#1]}
\newcommand{\ls}[1]{\ar@{-}[#1]}
\newcommand{\sj}[1]{\ar@{->>}[#1]}
\newcommand{\aq}[1]{\ar@{=}[#1]}
\newcommand{\acir}[1]{\ar@{}[#1]|-{\textstyle{\circlearrowright}}}
\newcommand{\acil}[1]{\ar@{}[#1]|-{\textstyle{\circlearrowleft}}}
\newcommand{\ard}[1]{\ar@{.>}[#1]}
\newcommand{\mt}[1]{\ar@{|->}[#1]}
\newcommand{\inm}[1]{\ar@{}[#1]|-{\in}}
\newcommand{\inr}{\ar@{}[d]|-{\rotatebox[origin=c]{-90}{$\in$}}}
\newcommand{\inl}{\ar@{}[u]|-{\rotatebox[origin=c]{90}{$\in$}}}

%Other
%\newcommand{\set}[2]{\left.\left\{{#1}\right|{#2}\right\}}
%\newcommand{\sett}[2]{\left\{{#1}\left|{#2}\right\}\right.}

%SUMS, ETC.
\newcommand{\sumr}[2]{\sum_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%sum with 2 rows
\newcommand{\prr}[2]{\prod_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\maxr}[2]{\max_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\minr}[2]{\min_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\trow}[2]{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}
\newcommand{\seqo}[3]{\{#3\}_{#1=1}^{#2}}
\newcommand{\su}[0]{\sum_{n=0}^{\iy}}
\newcommand{\suo}[0]{\sum_{n=1}^{\iy}}
\newcommand{\sumo}[2]{\sum_{#1=1}^{#2}}
\newcommand{\sumz}[2]{\sum_{#1=0}^{#2}}
\newcommand{\prodo}[2]{\prod_{#1=1}^{#2}}
\newcommand{\prodz}[2]{\prod_{#1=0}^{#2}}
\newcommand{\oplo}[2]{\bigopl_{#1=1}^{#2}}
\newcommand{\cupo}[2]{\bigcup_{#1=1}^{#2}}
\newcommand{\capo}[2]{\bigcap_{#1=1}^{#2}}
\newcommand{\iiy}[0]{\int_0^{\infty}}
\newcommand{\iny}[0]{\int_{-\infty}^{\infty}}
\newcommand{\iiiy}[0]{\int_{-\infty}^{\infty}}%DEPRECATED
\newcommand{\sui}[0]{\sum_{i=1}^{n}}
\newcommand{\suiy}[0]{\sum_{i=1}^{\iy}}
\newcommand{\cui}[0]{\bigcup_{i=1}^n}
\newcommand{\suj}[0]{\sum_{j=1}^{n}}
\newcommand{\suij}[0]{\sum_{i,j}}
\newcommand{\limn}[0]{\lim_{n\to \infty}}

%MATRICES

%Matrices
\newcommand{\scoltwo}[2]{
\left(\begin{smallmatrix}
{#1}\\
{#2}
\end{smallmatrix}\right)}
\newcommand{\coltwo}[2]{
\begin{pmatrix}
{#1}\\
{#2}
\end{pmatrix}}
\newcommand{\colthree}[3]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}
\end{pmatrix}
}
\newcommand{\colfour}[4]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}\\
{#4}
\end{pmatrix}
}
\newcommand{\cth}[3]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}
\end{pmatrix}
}
\newcommand{\detm}[4]{
\ab{
\begin{matrix}
{#1}&{#2}\\
{#3}&{#4}
\end{matrix}
}}
\newcommand{\sdetm}[4]{
\ab{
\begin{smallmatrix}
{#1}&{#2}\\
{#3}&{#4}
\end{smallmatrix}
}}
\newcommand{\matt}[4]{
\begin{pmatrix}
{#1}&{#2}\\
{#3}&{#4}
\end{pmatrix}
}
\newcommand{\smatt}[4]{
\left(\begin{smallmatrix} 
{#1}&{#2}\\
{#3}&{#4}
\end{smallmatrix}\right)
}
\newcommand{\mattn}[9]{
\begin{pmatrix}
{#1}&{#2}&{#3}\\
{#4}&{#5}&{#6}\\
{#7}&{#8}&{#9}
\end{pmatrix}
}
\newcommand{\smattn}[9]{
\left(\begin{smallmatrix}
{#1}&{#2}&{#3}\\
{#4}&{#5}&{#6}\\
{#7}&{#8}&{#9}
\end{smallmatrix}\right)
}

\newcommand{\bt}[2]{
\left\{\begin{matrix}
\text{#1}\\
\text{#2}
\end{matrix}
\right\}}
\newcommand{\bth}[3]{
\left\{\begin{matrix}
\text{#1}\\
\text{#2}\\
\text{#3}
\end{matrix}
\right\}}

\newcommand{\vvt}[1]{{#1}{#1}^\top}

\newcommand{\tcase}[4]{
\begin{cases}
#1 & #2\\
#3 & #4
\end{cases}}
\newcommand{\txcase}[4]{
\begin{cases}
#1 & \text{#2}\\
#3 & \text{#4}
\end{cases}}

\newcommand{\ifoth}[3]{
\begin{cases}
#1 & \text{if }#2\\
#3 & \text{otherwise}
\end{cases}}

%EQUATIONS
\newcommand{\beq}[1]{\begin{equation}\llabel{#1}}
\newcommand{\eeq}[0]{\end{equation}}
\newcommand{\bal}[0]{\begin{align*}}
\newcommand{\eal}[0]{\end{align*}}%this doesn't work; i don't know why
\newcommand{\ban}[0]{\begin{align}}
\newcommand{\ean}[0]{\end{align}}
\newcommand{\ig}[2]{\begin{center}\includegraphics[scale=#2]{#1}\end{center}}

%COURSE-SPECIFIC

%measure theory, analysis
\newcommand{\am}[0]{(a.e., $\mu$)}
\newcommand{\ftla}[1]{\int e^{i\lambda\cdot x}{#1}\,d\lambda}
\newcommand{\lime}[0]{\lim_{\varepsilon\to 0}}

%number theory
\newcommand{\modt}[1]{\,(\text{mod}^{\times}\, {#1})}
%\newcommand{\tl}[0]{T_{\ell}}
 %multiplicative subgroup
\newcommand{\zmod}[1]{\Z/{#1}\Z}
\newcommand{\md}[1]{\,(\text{mod }#1)}
%\newcommand{\ks}[1]{K(\sqrt{#1})}
\newcommand{\ksq}[1]{K(\sqrt{#1})/K}
\newcommand{\nksq}[1]{\nm_{K(\sqrt{#1})/K}(K(\sqrt{#1})^{\times})}
\newcommand{\mpp}[0]{\mP/\mfp}

%manifolds
\newcommand{\cvd}[0]{\frac{D}{\partial t}}
\newcommand{\cvs}[0]{\frac{D}{\partial s}}
\newcommand{\np}[1]{\nabla_{\pd{}{#1}}}

%algebraic geometry
%\newcommand{\av}[0]{A^{\vee}}


%arithmetic combinatorics
\newcommand{\Deq}[1]{\Delta^{\times}_{#1}}

%modular forms
\newcommand{\GLAi}[0]{\text{GL}_2(\mathbb A)_{\infty}}

%noise sensitivity part iii essay
\newcommand{\Dict}[0]{\operatorname{\mathsf{Dict}}}
\newcommand{\Maj}[0]{\operatorname{\mathsf{Maj}}}
\newcommand{\MAJ}[0]{\operatorname{\mathsf{Maj}}}
\newcommand{\Parity}[0]{\operatorname{\mathsf{Parity}}}
\newcommand{\Tribes}[0]{\operatorname{\mathsf{Tribes}}}
\newcommand{\Ns}[0]{\operatorname{NS}}
\newcommand{\DT}[0]{\operatorname{\mathsf{DT}}}
\newcommand{\DNF}[0]{\operatorname{\mathsf{DNF}}}
\newcommand{\CNF}[0]{\operatorname{\mathsf{CNF}}}
\newcommand{\Circuit}[0]{\operatorname{\mathsf{Circuit}}}
\newcommand{\Ac}[0]{\mathsf{AC}}
\newcommand{\EB}[0]{\text{EB}}
%comp complexity
%complexity theory
\newcommand{\ACC}[0]{\operatorname{\mathsf{ACC}}}
\newcommand{\BPP}[0]{\mathsf{BPP}}
\newcommand{\BPTIME}[0]{\operatorname{\mathsf{BPTIME}}}
\newcommand{\CLIQUE}[0]{\operatorname{\mathsf{CLIQUE}}}
\newcommand{\EXP}[0]{\mathsf{EXP}}
\newcommand{\NEXP}[0]{\mathsf{NEXP}}
\newcommand{\NC}[0]{\operatorname{\mathsf{NC}}}
\newcommand{\NP}[0]{\operatorname{\mathsf{NP}}}
\newcommand{\NTIME}[0]{\operatorname{\mathsf{NTIME}}}
\newcommand{\msP}[0]{\operatorname{\mathsf{P}}}
\newcommand{\PCP}[0]{\operatorname{\mathsf{PCP}}}
\newcommand{\SAT}[0]{\mathsf{SAT}}
\newcommand{\SUBEXP}[0]{\mathsf{SUBEXP}}
\newcommand{\TIME}[0]{\operatorname{\mathsf{TIME}}}
\newcommand{\zz}{\textcircled{Z}}
%statistics
\newcommand{\hten}[0]{\widehat{\theta_n}}

%EDITING HELP
%blu: key idea or concept. red: unresolved issue/question. 
\newcommand{\blu}[1]{{\color{blue}#1}}
\newcommand{\grn}[1]{{\color{green}#1}}
\newcommand{\redd}[1]{{\color{red}#1}}
\newcommand{\pur}[1]{{\color{purple}#1}}
\newcommand{\oge}[1]{{\color{orange}#1}}
\newcommand{\concept}[1]{#1}
\newcommand{\fixme}[1]{{\color{red}#1}}
\newcommand{\cary}[1]{{\color{purple}#1}}%deprecated
%short for commentary
\newcommand{\llabel}[1]{\label{#1}\text{\fixme{\tiny#1}}}
\newcommand{\nref}[1]{\ref{#1}}
%%%%%%%%%%%
%Use the above when working on the document, so labels will be displayed by their theorems, and you can write reminders to yourself. Switch to the below commands when publishing.
%%%%%%%%%%%
%\newcommand{\fixme}[1]{}
%\newcommand{\concept}[1]{{\color{blue}#1}}
%\newcommand{\llabel}[1]{\label{#1}}
%%%%%%%%%%%

\newcommand{\itag}[1]{\index{#1}[\##1]}
\newcommand{\ilbl}[1]{[#1]\index{#1}}
\newcommand{\iadd}[1]{\index{#1} #1}
\newcommand{\arxiv}[1]{\url{http://www.arxiv.org/abs/#1}}

%markup
\newcommand{\ivocab}[1]{\index{#1}\textbf{#1}}
\newcommand{\vocab}[1]{\textbf{#1}} %also index automatically.
\newcommand{\summq}[1]{\textbf{Summary Question: }#1}
\newcommand{\keypt}[1]{{\it #1}}
\newcommand{\subprob}[1]{\noindent\textbf{#1}\\}
\newcommand{\qatable}[1]{\begin{center}
    \begin{longtable}{ | p{5.5cm} | p{10cm} |}
#1
\end{longtable}
\end{center}}

%%Newcommands
%k'
\newcommand{\kp}[0]{\fl{d\log_2(M)}}
%(2/ln 2)d
\newcommand{\Lad}[0]{\fc{2}{\ln 2}d}
\newcommand{\Ladm}[0]{\fc{2}{\ln 2}(d+m)}
\newcommand{\Laldm}[0]{\fc{2}{\ln 2}\ell(d+m)}
%B_{(2/ln 2)d}^d
\newcommand{\Bd}[0]{B_{\Lad}^d}
%K_0\cup B_{(2/ln 2)d}^d
\newcommand{\KuB}[0]{K_0\cup B_{\Lad}^d}
%L_v
\newcommand{\Lvg}[0]{\max_{0\le k\le k'} f_{A,\KuB}(k) +  \pa{\sumz k{k'-1}f_{A,K}(k)} \pa{\Lad+1}}
%\max{(2/ln 2)d,C_0}
\newcommand{\maxdc}[0]{\max\bc{\fc{2}{\ln 2}d,C_0}}
%L_v(p)
\newcommand{\Lp}[0]{\max_{0\le k\le p(k'+1)-1} f_A(k)\maxdc
+ \pa{\sumz k{p(k'+1)-2} f_{A,K}(k)}\pa{\Lad+2}}
\newcommand{\maxprederrorJ}[0]{\max\bc{
\fc{C_\xi c^2t}{\mu}+ac, \fc{C_\xi}{c_2^2}, \rc{c_1^{\fc 1{\al+2}}c_2^{\fc 2{\al+2}}}\pa{a\mu^{\fc{1}{\al+2}} + \fc{C_\xi t^{\rc 2}}{\mu^{\rc2-\rc{\al+2}}}}
}}
\newcommand{\maxprederrorJA}[0]{\max\bc{
\fc{C_\xi c^2t}{\mu}+\ve{A}_2c, \fc{C_\xi}{c_2^2}, \rc{c_1^{\fc 1{\al+2}}c_2^{\fc 2{\al+2}}}\pa{\ve{A}_2\mu^{\fc{1}{\al+2}} + \fc{C_\xi t^{\rc 2}}{\mu^{\rc2-\rc{\al+2}}}}
}}
\newcommand{\maxprederrorJAT}[0]{\max\bc{
\fc{C_\xi c^2T}{\mu}+\ve{(A,B)}_2c, \fc{C_\xi}{c_2^2}, \rc{c_1^{\fc 1{\al+2}}c_2^{\fc 2{\al+2}}}\pa{\ve{(A,B)}_2\mu^{\fc{1}{\al+2}} + \fc{C_\xi T^{\rc 2}}{\mu^{\rc2-\rc{\al+2}}}}
}}
%k'(d+m)
\newcommand{\kdm}[0]{\fl{(d+m)\log_2(M)}}
\newcommand{\kldm}[0]{\fl{\ell(d+m)\log_2(M)}}
%\newcommand{\LpAB}[0]{(p(k'+1))^{r-1} \maxdmc +  [C r(p(k'+1))^r+C_u] \pa{\Ladm+2}}
\newcommand{\clbd}[0]{2^{r+1}C(k'+1)^r \pa{\Ladm(C+1)+C_0+2}+4C_u\pa{\Ladm+2}}
\newcommand{\Mbd}[0]{(T+1)^{r-1} C_AC_0+T^r C_A(C_BC_u+C_\xi)}
\newcommand{\maxdmc}[0]{\max\bc{\fc{2}{\ln 2}(d+m),C_0}}

\newcommand{\ctzz}[2]{\pa{
\begin{array}{c}
#1\\
\mathbf 0\\
\hline
#2\\
\mathbf 0
\end{array}
}}



%Page breaks in equations
\allowdisplaybreaks[2]

%SHA
\DeclareFontFamily{U}{wncy}{}
    \DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
    \DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
    \DeclareMathSymbol{\Sh}{\mathord}{mcy}{"58} 

==> format/macros.tex <==
%authornote
\def\shownotes{1}  \ifnum\shownotes=1
\newcommand{\authnote}[2]{$\ll$\textsf{\footnotesize #1 notes: #2}$\gg$}
\else
\newcommand{\authnote}[2]{}
\fi
\newcommand{\hlnote}[1]{{\color{purple}\authnote{HL}{#1}}}

\newcommand{\st}[0]{\mathscr{st}}

%LETTERS

%UPPERCASE
\newcommand{\KL}[0]{\operatorname{KL}}
\newcommand{\sA}[0]{\mathscr{A}}
\newcommand{\cA}[0]{\mathcal{A}}
%\newcommand{\A}[0]{\mathbb{A}}
\newcommand{\cB}[0]{\mathcal{B}}
%\newcommand{\C}[0]{\mathbb{C}}
\newcommand{\sC}[0]{\mathcal{C}}%deprecated
\newcommand{\cC}[0]{\mathcal{C}}
\newcommand{\sD}[0]{\mathscr{D}}
\newcommand{\mD}[0]{\mathfrak D}
\newcommand{\cE}[0]{\mathscr{E}}%deprecated
\newcommand{\sE}[0]{\mathscr{E}}
%\newcommand{\E}[0]{\mathbb{E}}
\newcommand{\EE}[0]{\mathop{\mathbb E}}
%\scalebox{1.25}{$\mathbb E$}}
\newcommand{\F}[0]{\mathbb{F}}
\newcommand{\cF}[0]{\mathscr{F}}%deprecated.
\newcommand{\sF}[0]{\mathscr{F}}
%\newcommand{\G}[0]{\mathbb{G}}
\newcommand{\cG}[0]{\mathscr{G}}%deprecated.
\newcommand{\sG}[0]{\mathscr{G}}
%\newcommand{\cH}[0]{\mathcal H}%deprecated
\newcommand{\sH}[0]{\mathscr H}
\newcommand{\Hq}[0]{\mathbb{H}}
\newcommand{\bfI}[0]{\mathbf{I}}
\newcommand{\I}[0]{\mathbb{I}}
\newcommand{\cI}[0]{\mathscr{I}}%deprecated
\newcommand{\sI}[0]{\mathscr{I}}
\newcommand{\cJ}[0]{\mathscr{J}}
\newcommand{\cL}[0]{\mathscr{L}}
%\newcommand{\N}[0]{\mathbb{N}}
\newcommand{\fN}[0]{\mathfrak{N}}
\newcommand{\cP}[0]{\mathcal{P}}
\newcommand{\Pj}[0]{\mathbb{P}}
%\newcommand{\mP}[0]{\mathfrak{P}}
\newcommand{\mQ}[0]{\mathfrak{Q}}
%!
\newcommand{\cO}[0]{\mathcal{O}}
\newcommand{\sO}[0]{\mathscr{O}}
\newcommand{\Q}[0]{\mathbb{Q}}
%\newcommand{\R}[0]{\mathbb{R}}
%\newcommand{\bS}[0]{\mathbb{S}}
\newcommand{\T}[0]{\mathbb{T}}
%\newcommand{\X}[0]{\mathfrak{X}}
\newcommand{\Z}[0]{\mathbb{Z}}
\newcommand{\one}[0]{\mathbbm{1}}
%lowercase
\newcommand{\mba}[0]{\mathbf{a}}%idele a
\newcommand{\ma}[0]{\mathfrak{a}}%ideal a
\newcommand{\mb}[0]{\mathfrak{b}}
\newcommand{\mc}[0]{\mathfrak{c}}
\newcommand{\mfd}[0]{\mathfrak d}
\newcommand{\mf}[0]{\mathfrak{f}}
\newcommand{\fg}[0]{\mathfrak{g}}
\newcommand{\vi}[0]{\mathbf{i}}%vector i
\newcommand{\vj}[0]{\mathbf{j}}
\newcommand{\vk}[0]{\mathbf{k}}
\newcommand{\mm}[0]{\mathfrak{m}}%ideal m
\newcommand{\mfp}[0]{\mathfrak{p}}
\newcommand{\mq}[0]{\mathfrak{q}}
\newcommand{\mr}[0]{\mathfrak{r}}
\newcommand{\mv}[0]{\mathbf{v}}
\newcommand{\mx}[0]{\mathbf{x}}%idele x
\newcommand{\my}[0]{\mathbf{y}}
%More sequences of letters
\newcommand{\et}[0]{_{\text{\'et}}}
\newcommand{\Gm}[0]{\mathbb{G}_m}
\newcommand{\Fp}[0]{\mathbb{F}_p}
\newcommand{\fq}[0]{\mathbb{F}_q}
\newcommand{\fpb}[0]{\ol{\mathbb{F}_p}}
\newcommand{\fpt}[0]{\mathbb{F}_p^{\times}}
\newcommand{\fqt}[0]{\mathbb{F}_q^{\times}}
\newcommand{\Kt}[0]{K^{\times}}
\newcommand{\RP}[0]{\mathbb{R}P}
\newcommand{\qb}[0]{\ol{\mathbb{Q}}}
\newcommand{\qp}[0]{\mathbb{Q}_p}
\newcommand{\qpb}[0]{\ol{\mathbb{Q}_p}}
\newcommand{\ql}[0]{\mathbb Q_{\ell}}
\newcommand{\sll}[0]{\mathfrak{sl}}
\newcommand{\vl}[0]{V_{\ell}}
\newcommand{\zl}[0]{\mathbb Z_{\ell}}
\newcommand{\zp}[0]{\mathbb Z_{p}}
\newcommand{\zpz}[0]{\mathbb Z/p\mathbb Z}
%Shortcuts for greek letters
\newcommand{\al}[0]{\alpha}
\newcommand{\be}[0]{\beta}
\newcommand{\ga}[0]{\gamma}
\newcommand{\Ga}[0]{\Gamma}
\newcommand{\de}[0]{\delta}
\newcommand{\De}[0]{\Delta}
\newcommand{\ep}[0]{\varepsilon}
\newcommand{\eph}[0]{\frac{\varepsilon}{2}}
\newcommand{\ept}[0]{\frac{\varepsilon}{3}}
\newcommand{\ka}[0]{\kappa}
\newcommand{\la}[0]{\lambda}
\newcommand{\La}[0]{\Lambda}
\newcommand{\ph}[0]{\varphi}
\newcommand{\Ph}[0]{\Phi}
\newcommand{\rh}[0]{\rho}
\newcommand{\te}[0]{\theta}
\newcommand{\Te}[0]{\Theta}
\newcommand{\vte}[0]{\vartheta}
\newcommand{\om}[0]{\omega}
\newcommand{\Om}[0]{\Omega}
\newcommand{\si}[0]{\sigma}
\newcommand{\Si}[0]{\Sigma}
\newcommand{\ze}[0]{\zeta}

%SYMBOLS

%Shortcuts for symbols
\newcommand{\nin}[0]{\not\in}
\newcommand{\opl}[0]{\oplus}
\newcommand{\bigopl}[0]{\bigoplus}
\newcommand{\ot}[0]{\otimes}
\newcommand{\bigot}[0]{\bigotimes}
\newcommand{\sub}[0]{\subset}
\newcommand{\nsub}[0]{\not\subset}
\newcommand{\subeq}[0]{\subseteq}
\newcommand{\supeq}[0]{\supseteq}
\newcommand{\nsubeq}[0]{\not\subseteq}
\newcommand{\nsupeq}[0]{\not\supseteq}
\newcommand{\nequiv}[0]{\not\equiv}
\newcommand{\bs}[0]{\backslash}
\newcommand{\iy}[0]{\infty}
\newcommand{\no}[0]{\trianglelefteq}%normal subgroup
\newcommand{\qeq}[0]{\stackrel?=}
\newcommand{\subsim}[0]{\stackrel{\sub}{\sim}}
\newcommand{\supsim}[0]{\stackrel{\supset}{\sim}}
\newcommand{\na}[0]{\nabla}
\newcommand{\mcv}[0]{*_-}
\newcommand{\dlim}[0]{\varinjlim}
\newcommand{\ilim}[0]{\varprojlim}
\newcommand{\gle}[0]{\begin{array}{c}
\ge\\
\le
\end{array}}
\newcommand{\lge}[0]{\begin{array}{c}
\le\\
\ge
\end{array}}
%\stackrel{-}{*}}%minus convoluion.

%COMMON TIME-SAVERS

%Fractions
\newcommand{\rc}[1]{\frac{1}{#1}}
\newcommand{\prc}[1]{\pa{\rc{#1}}}
\newcommand{\ff}[2]{\left\lfloor\frac{#1}{#2}\right\rfloor}
\newcommand{\cf}[2]{\left\lceil\frac{#1}{#2}\rceil\rfloor}
\newcommand{\fc}[2]{\frac{#1}{#2}}
\newcommand{\sfc}[2]{\sqrt{\frac{#1}{#2}}}
\newcommand{\pf}[2]{\pa{\frac{#1}{#2}}}%Shortcut for fraction with parentheses
\DeclareRobustCommand{\stl}{\genfrac\{\}{0pt}{}}

\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}%Partial derivatives
\newcommand{\dd}[2]{\frac{d #1}{d #2}}
\newcommand{\pdd}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ddd}[1]{\frac{d}{d #1}}
\newcommand{\af}[2]{\ab{\fc{#1}{#2}}}
\newcommand{\ddt}[2]{\frac{d^2 #1}{d {#2}^2}}
\newcommand{\pdt}[2]{\frac{\partial^2 #1}{\partial {#2}^2}}
\newcommand{\pdxy}[3]{\frac{\partial^2 #1}{\partial {#2}\partial {#3}}}
\newcommand{\pl}[0]{\partial}
\newcommand{\nb}[0]{\nabla}
\newcommand{\onb}[0]{\ol{\nabla}}
\newcommand{\dy}{\,dy}
\newcommand{\dx}{\,dx}

%Arrows
\newcommand{\lar}[0]{\leftarrow}
\newcommand{\ra}[0]{\rightarrow}
\newcommand{\dra}[0]{\dashrightarrow}
\newcommand{\lra}[0]{\leftrightarrow}
\newcommand{\rra}[0]{\twoheadrightarrow}
\newcommand{\hra}[0]{\hookrightarrow}
\newcommand{\tra}[0]{\twoheadrightarrow}
\newcommand{\send}[0]{\mapsto}
\newcommand{\xra}[1]{\xrightarrow{#1}}
\newcommand{\xla}[1]{\xleftarrow{#1}}
\newcommand{\xhra}[1]{\xhookrightarrow{#1}}
\newcommand{\xlra}[1]{\xleftrightarrow{#1}}
\newcommand{\xrc}[0]{\xrightarrow{\cong}}
%\renewcommand{\cir}[0]{\circlearrowright}
\newcommand{\cil}[0]{\circlearrowleft}

%Brackets
\newcommand{\ab}[1]{\left| {#1} \right|}
\newcommand{\an}[1]{\left\langle {#1}\right\rangle}
\newcommand{\ba}[1]{\left[ {#1} \right]}
\newcommand{\bc}[1]{\left\{ {#1} \right\}}
%\newcommand{\bra}[1]{\langle{#1}|}
\newcommand{\braa}[1]{\langle\langle{#1}|}
\newcommand{\ce}[1]{\left\lceil {#1}\right\rceil}
\newcommand{\fl}[1]{\left\lfloor {#1}\right\rfloor}
\newcommand{\ro}[1]{\left\lfloor {#1}\right\rceil}
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\kett}[1]{|{#1}\rangle\rangle}
%\newcommand{\bk}[2]{\langle{#1}|{#2}\rangle}
\newcommand{\braak}[2]{\langle\langle{#1}|{#2}\rangle\rangle}
\newcommand{\kbb}[1]{|{#1}\rangle\langle{#1}|}
\newcommand{\kb}[2]{|{#1}\rangle\langle{#2}|}
\newcommand{\kettb}[2]{|{#1}\rangle\rangle\langle\langle{#2}|}
\newcommand{\pa}[1]{\left( {#1} \right)}
\newcommand{\pat}[1]{\left( \text{#1} \right)}
\newcommand{\ve}[1]{\left\Vert {#1}\right\Vert}
\newcommand{\nv}[1]{\frac{#1}{\left\Vert {#1}\right\Vert}}
\newcommand{\nvl}[2]{\frac{#1}{\left\Vert {#1}\right\Vert_{#2}}}
\newcommand{\rb}[1]{\left.{#1}\right|}
%\newcommand{\nl}[1]{\left\Vert #1 \right\Vert_{L^1}}
\newcommand{\ad}[0]{|\cdot|}
\newcommand{\ved}[0]{\ve{\cdot}}
\newcommand{\set}[2]{\left\{{#1}:{#2}\right\}}
\newcommand{\sett}[2]{\left\{\left.{#1}\right|{#2}\right\}}

%under and overlines, etc.
\newcommand{\ch}[1]{\check{#1}}
\newcommand{\dch}[1]{\check{\check{#1}}}
\newcommand{\olra}[1]{\overleftrightarrow{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ub}[2]{\underbrace{#1}_{#2}}
\newcommand{\ora}[1]{\overrightarrow{#1}}
\newcommand{\ura}[1]{\underrightarrow{#1}}
%\newcommand{\wt}[1]{\widetilde{#1}}
%\newcommand{\wh}[1]{\widehat{#1}}

%other
\newcommand{\fp}[1]{^{\underline{#1}}}%Falling power
\newcommand{\rp}[1]{^{\overline{#1}}}
\newcommand{\pp}[1]{^{(#1)}}
\newcommand{\sh}[0]{^{\sharp}}
\newcommand{\ri}[0]{\ddagger}%replace this with rosati involution
\newcommand{\bit}[0]{\{0,1\}}

%TEXT
\newcommand{\btih}[1]{\text{ by the induction hypothesis{#1}}}
\newcommand{\bwoc}[0]{by way of contradiction}
%\newcommand{\by}[1]{\text{by~(\ref{#1})}}
\newcommand{\idk}[0]{{\color{red}I don't know.} }
\newcommand{\ore}[0]{\text{ or }}
\newcommand{\wog}[0]{ without loss of generality }
\newcommand{\Wog}[0]{ Without loss of generality }
\newcommand{\step}[1]{\noindent{\underline{Step {#1}:}}}
\newcommand{\prt}[1]{\noindent{\underline{Part {#1}:}}}
\newcommand{\tfae}[0]{ the following are equivalent}
\newcommand{\fabfm}[0]{for all but finitely many }

%FUNCTIONS
%Functions, etc.
\newcommand{\Abs}{(\text{Ab}/S)}
\newcommand{\abk}{(\text{Ab}/k)}
\newcommand{\abc}{(\text{Ab}/\C)}
\newcommand{\Alb}{\operatorname{Alb}}
\newcommand{\Ann}{\operatorname{Ann}}
\newcommand{\Area}{\operatorname{Area}}
\newcommand{\amax}{\operatorname{argmax}}
\newcommand{\amin}{\operatorname{argmin}}
\newcommand{\Ass}{\operatorname{Ass}}
\newcommand{\Art}{\operatorname{Art}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\avg}{\operatorname{avg}}
%\newcommand{\bias}[0]{\operatorname{bias}}
\newcommand{\Binom}{\operatorname{Binom}}
\newcommand{\Bl}[0]{\operatorname{Bl}}
\newcommand{\Br}{\operatorname{Br}}
\newcommand{\chr}{\operatorname{char}}
\newcommand{\cis}{\operatorname{cis}}
\newcommand{\cl}{\operatorname{Cl}}
%\newcommand{\Cl}{C}%changed notation%this is confusing
\newcommand{\Cl}{\operatorname{Cl}}
\newcommand{\Coh}{\operatorname{Coh}}
\newcommand{\Coinf}[0]{\operatorname{Coinf}}
\newcommand{\Coind}[0]{\operatorname{Coind}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\colim}{\operatorname{colim}}
\newcommand{\Comp}{\operatorname{Comp}}
%\newcommand{\conv}{\operatorname{conv}}
\newcommand{\oconv}{\ol{\conv}}
\newcommand{\Cor}{\operatorname{Cor}}
%\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\cro}{\operatorname{cr}}
\newcommand{\degs}[0]{\deg_{\text{s}}}%separable degree
\newcommand{\Dec}{\operatorname{Dec}}
\newcommand{\depth}{\operatorname{depth}}
\newcommand{\Der}{\operatorname{Der}}
%\newcommand{\diag}{\operatorname{diag}}
\newcommand{\diam}{\operatorname{diam}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\Dir}{\operatorname{Dir}}
\newcommand{\Div}{\operatorname{Div}}
\newcommand{\Disc}{\operatorname{Disc}}%discrepancy
\newcommand{\disc}{\operatorname{disc}}%discriminant
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\Ell}{\mathcal{E}{\rm{ll}}}
\newcommand{\Enc}{\operatorname{Enc}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Ent}{\operatorname{Ent}}
\newcommand{\Ext}{\operatorname{Ext}}
%\newcommand{\Exp}{\operatorname{Exp}}
\newcommand{\err}{\operatorname{err}}
\newcommand{\ess}{\operatorname{ess}}
\newcommand{\ext}{\operatorname{ext}}
\newcommand{\pfcg}{(p\text{-FCGp}/k)}
\newcommand{\fcg}{(\text{FCGp}/k)}
\newcommand{\Frac}{\operatorname{Frac}}
\newcommand{\Frob}{\operatorname{Frob}}
\newcommand{\Fun}{\operatorname{Fun}}
\newcommand{\FS}{\operatorname{FS}}
\newcommand{\Gal}{\operatorname{Gal}}
\newcommand{\Gap}{\operatorname{Gap}}
%\newcommand{\grad}{\operatorname{grad}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\gps}{(\text{Gp}/S)}
\newcommand{\Hess}{\operatorname{Hess}}
\newcommand{\Het}{H_{\text{\'et}}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Homeo}{\operatorname{Homeo}}
\newcommand{\chom}[0]{\mathscr{H}om}
\newcommand{\Homc}{\operatorname{Hom}_{\text{cont}}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\im}[0]{\text{im}}
\newcommand{\imp}[0]{\im^{\text{pre}}}
\newcommand{\Ind}[0]{\operatorname{Ind}}
\newcommand{\Inf}[0]{\operatorname{Inf}}
\newcommand{\inv}[0]{\operatorname{inv}}
\newcommand{\Isoc}[0]{\operatorname{Isoc}}
\newcommand{\Isog}[0]{\operatorname{Isog}}
\newcommand{\Isom}[0]{\operatorname{Isom}}
\newcommand{\Jac}[0]{\operatorname{Jac}}
\newcommand{\li}[0]{\operatorname{li}}
\newcommand{\Li}[0]{\operatorname{li}}
\newcommand{\Lie}[0]{\operatorname{Lie}}
\newcommand{\Line}[0]{\operatorname{Line}}
\newcommand{\Lip}[0]{\operatorname{Lip}}
\newcommand{\lcm}[0]{\operatorname{lcm}}
\newcommand{\Mat}{\operatorname{Mat}}
\newcommand{\Mod}{\operatorname{Mod}}
\newcommand{\Dmod}{\Mod_{W[F,V]}^{\text{fl}}}
\newcommand{\nil}[0]{\operatorname{nil}}
\newcommand{\nm}{\operatorname{Nm}}
\newcommand{\NS}{\operatorname{NS}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\PDer}{\operatorname{PDer}}
\newcommand{\PGL}{\operatorname{PGL}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Pico}{\operatorname{Pic}^{\circ}}
\newcommand{\Pois}{\operatorname{Pois}}
%\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\PSL}{\operatorname{PSL}}
\newcommand{\Per}{\operatorname{Per}}
\newcommand{\perm}{\operatorname{perm}}
\newcommand{\PrePer}{\operatorname{PrePer}}
\newcommand{\Prob}{\operatorname{Prob}}
\newcommand{\Proj}{\operatorname{Proj}}
\newcommand{\Prj}[0]{\textbf{Proj}}
\newcommand{\QCoh}{\operatorname{QCoh}}
\newcommand{\Rad}{\operatorname{Rad}}
\newcommand{\range}{\operatorname{range}}
%\newcommand{\rank}{\operatorname{rank}}
\newcommand{\red}{\operatorname{red}}
\newcommand{\Reg}{\operatorname{Reg}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\Ric}{\operatorname{Ric}} %Ricci curvature
\newcommand{\rot}{\operatorname{rot}}
\newcommand{\Scal}{\operatorname{Scal}} %Ricci curvature
\newcommand{\schs}{(\text{Sch}/S)}
\newcommand{\schk}{(\text{Sch}/k)}
\newcommand{\se}{\text{se}}
\newcommand{\srank}{\text{srank}}
\newcommand{\hse}{\wh{\text{se}}}
\newcommand{\Sel}{\operatorname{Sel}}
\newcommand{\sens}{\operatorname{sens}}
\newcommand{\Set}{(\text{Set})}
%\newcommand{\sgn}{\operatorname{sign}}
%\newcommand{\sign}{\operatorname{sign}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\Specf}[2]{\Spec\pa{\frac{k[{#1}]}{#2}}}
\newcommand{\rspec}{\ul{\operatorname{Spec}}}
\newcommand{\Spl}{\operatorname{Spl}}
\newcommand{\spp}{\operatorname{sp}}
%\newcommand{\spn}{\operatorname{span}}
\newcommand{\Stab}{\operatorname{Stab}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\ssupp}{\operatorname{sing}\operatorname{supp}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\Th}{\operatorname{Th}}
\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\tor}{\operatorname{tor}}
\newcommand{\Tr}[0]{\operatorname{Tr}}
%\newcommand{\tr}[0]{\operatorname{tr}}
%\newcommand{\val}[0]{\text{val}}
%\newcommand{\Var}[0]{\operatorname{Var}}
%\newcommand{\var}[0]{\text{var}}
\newcommand{\vcong}{\operatorname{vcong}}
\newcommand{\Vol}[0]{\text{Vol}}
%\newcommand{\vol}[0]{\text{vol}}
\providecommand{\cal}[1]{\mathcal{#1}}
\renewcommand{\cal}[1]{\mathcal{#1}}
\providecommand{\bb}[1]{\mathbb{#1}}
\renewcommand{\bb}[1]{\mathbb{#1}}

%Text super/subscripts
\newcommand{\abe}[0]{^{\text{ab}}}
\newcommand{\gal}[0]{^{\text{gal}}}%galois closure
\newcommand{\op}{^{\text{op}}}
\newcommand{\pre}[0]{^{\text{pre}}}
\newcommand{\rd}[0]{_{\text{red}}}
\newcommand{\sep}[0]{^{\text{sep}}}
\newcommand{\tp}{^{\text{top}}}
\newcommand{\tors}{_{\text{tors}}}
\newcommand{\ur}[0]{^{\text{ur}}}
\newcommand{\urt}[0]{^{\text{ur}\times}}

%COMMUTATIVE DIAGRAMS

%Commutative diagram shortcuts
\newcommand{\commsq}[8]{\xymatrix{#1\ar[r]^-{#6}\ar[d]_{#5} &#2\ar[d]^{#7} \\ #3 \ar[r]^-{#8} & #4}}
%Makes a diagram like this
%1->2
%|    |
%3->4
%Arguments 5, 6, 7, 8 on arrows
%  6
%5  7
%  8
\newcommand{\pull}[9]{
#1\ar@/_/[ddr]_{#2} \ar@{.>}[rd]^{#3} \ar@/^/[rrd]^{#4} & &\\
& #5\ar[r]^{#6}\ar[d]^{#8} &#7\ar[d]^{#9} \\}
\newcommand{\back}[3]{& #1 \ar[r]^{#2} & #3}
%Syntax:\pull 123456789 \back ABC
%1=upper left-hand corner
%2,3,4=arrows from upper LH corner, going down, diagonal, right
%5,6,7=top row (6 on arrow)
%8,9=middle rows (on arrows)
%A,B,C=bottom row
%composition
\newcommand{\cmp}[9]{
\xymatrix{
#1 \ar[r]^{#4}{#5} \ar@/_2pc/[rr]^{#8}_{#9} & #2 \ar[r]^{#6}_{#7} & #3
}
}
\newcommand{\ctr}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5}\ar[rd]^{#6}_{#7} && #2\ar[ld]_{#8}^{#9}\\
& #3 &
}
}
\newcommand{\ctrr}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5} && #2\\
& #3 \ar[lu]_{#6}^{#7}\ar[ru]_{#8}^{#9}&
}
}

\newcommand{\ctri}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5}\ar[rd]^{#6}_{#7} && #2\\
& #3 \ar[ru]^{#8}_{#9}&
}
}
\newcommand{\rcommsq}[8]{\xymatrix{#1 &#2\ar[l]_-{#6} \\ #3 \ar[u]^{#5} & #4 \ar[u]_{#7}\ar[l]_-{#8}}}


%Arrow shortcuts
\newcommand{\ha}[1]{\ar@{^(->}[#1]}
\newcommand{\ls}[1]{\ar@{-}[#1]}
\newcommand{\sj}[1]{\ar@{->>}[#1]}
\newcommand{\aq}[1]{\ar@{=}[#1]}
\newcommand{\acir}[1]{\ar@{}[#1]|-{\textstyle{\circlearrowright}}}
\newcommand{\acil}[1]{\ar@{}[#1]|-{\textstyle{\circlearrowleft}}}
\newcommand{\ard}[1]{\ar@{.>}[#1]}
\newcommand{\mt}[1]{\ar@{|->}[#1]}
\newcommand{\inm}[1]{\ar@{}[#1]|-{\in}}
\newcommand{\inr}{\ar@{}[d]|-{\rotatebox[origin=c]{-90}{$\in$}}}
\newcommand{\inl}{\ar@{}[u]|-{\rotatebox[origin=c]{90}{$\in$}}}

%Other
%\newcommand{\set}[2]{\left.\left\{{#1}\right|{#2}\right\}}
%\newcommand{\sett}[2]{\left\{{#1}\left|{#2}\right\}\right.}

%SUMS, ETC.
\newcommand{\sumr}[2]{\sum_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%sum with 2 rows
\newcommand{\prr}[2]{\prod_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\maxr}[2]{\max_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\minr}[2]{\min_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\trow}[2]{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}
\newcommand{\seqo}[3]{\{#3\}_{#1=1}^{#2}}
\newcommand{\su}[0]{\sum_{n=0}^{\iy}}
\newcommand{\suo}[0]{\sum_{n=1}^{\iy}}
\newcommand{\sumo}[2]{\sum_{#1=1}^{#2}}
\newcommand{\sumz}[2]{\sum_{#1=0}^{#2}}
\newcommand{\prodo}[2]{\prod_{#1=1}^{#2}}
\newcommand{\prodz}[2]{\prod_{#1=0}^{#2}}
\newcommand{\oplo}[2]{\bigopl_{#1=1}^{#2}}
\newcommand{\cupo}[2]{\bigcup_{#1=1}^{#2}}
\newcommand{\capo}[2]{\bigcap_{#1=1}^{#2}}
\newcommand{\iiy}[0]{\int_0^{\infty}}
\newcommand{\iny}[0]{\int_{-\infty}^{\infty}}
\newcommand{\iiiy}[0]{\int_{-\infty}^{\infty}}%DEPRECATED
\newcommand{\sui}[0]{\sum_{i=1}^{n}}
\newcommand{\suiy}[0]{\sum_{i=1}^{\iy}}
\newcommand{\cui}[0]{\bigcup_{i=1}^n}
\newcommand{\suj}[0]{\sum_{j=1}^{n}}
\newcommand{\suij}[0]{\sum_{i,j}}
\newcommand{\limn}[0]{\lim_{n\to \infty}}

%MATRICES

%Matrices
\newcommand{\scoltwo}[2]{
\left(\begin{smallmatrix}
{#1}\\
{#2}
\end{smallmatrix}\right)}
\newcommand{\coltwo}[2]{
\begin{pmatrix}
{#1}\\
{#2}
\end{pmatrix}}
\newcommand{\colthree}[3]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}
\end{pmatrix}
}
\newcommand{\colfour}[4]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}\\
{#4}
\end{pmatrix}
}
\newcommand{\cth}[3]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}
\end{pmatrix}
}
\newcommand{\detm}[4]{
\ab{
\begin{matrix}
{#1}&{#2}\\
{#3}&{#4}
\end{matrix}
}}
\newcommand{\sdetm}[4]{
\ab{
\begin{smallmatrix}
{#1}&{#2}\\
{#3}&{#4}
\end{smallmatrix}
}}
\newcommand{\matt}[4]{
\begin{pmatrix}
{#1}&{#2}\\
{#3}&{#4}
\end{pmatrix}
}
\newcommand{\smatt}[4]{
\left(\begin{smallmatrix} 
{#1}&{#2}\\
{#3}&{#4}
\end{smallmatrix}\right)
}
\newcommand{\mattn}[9]{
\begin{pmatrix}
{#1}&{#2}&{#3}\\
{#4}&{#5}&{#6}\\
{#7}&{#8}&{#9}
\end{pmatrix}
}
\newcommand{\smattn}[9]{
\left(\begin{smallmatrix}
{#1}&{#2}&{#3}\\
{#4}&{#5}&{#6}\\
{#7}&{#8}&{#9}
\end{smallmatrix}\right)
}

\newcommand{\bt}[2]{
\left\{\begin{matrix}
\text{#1}\\
\text{#2}
\end{matrix}
\right\}}
\newcommand{\bth}[3]{
\left\{\begin{matrix}
\text{#1}\\
\text{#2}\\
\text{#3}
\end{matrix}
\right\}}

\newcommand{\vvt}[1]{{#1}{#1}^\top}

\newcommand{\tcase}[4]{
\begin{cases}
#1 & #2\\
#3 & #4
\end{cases}}
\newcommand{\txcase}[4]{
\begin{cases}
#1 & \text{#2}\\
#3 & \text{#4}
\end{cases}}

\newcommand{\ifoth}[3]{
\begin{cases}
#1 & \text{if }#2\\
#3 & \text{otherwise}
\end{cases}}

%EQUATIONS
\newcommand{\beq}[1]{\begin{equation}\llabel{#1}}
\newcommand{\eeq}[0]{\end{equation}}
\newcommand{\bal}[0]{\begin{align*}}
\newcommand{\eal}[0]{\end{align*}}%this doesn't work; i don't know why
\newcommand{\ban}[0]{\begin{align}}
\newcommand{\ean}[0]{\end{align}}
\newcommand{\ig}[2]{\begin{center}\includegraphics[scale=#2]{#1}\end{center}}

%COURSE-SPECIFIC

%measure theory, analysis
\newcommand{\am}[0]{(a.e., $\mu$)}
\newcommand{\ftla}[1]{\int e^{i\lambda\cdot x}{#1}\,d\lambda}
\newcommand{\lime}[0]{\lim_{\varepsilon\to 0}}

%number theory
\newcommand{\modt}[1]{\,(\text{mod}^{\times}\, {#1})}
%\newcommand{\tl}[0]{T_{\ell}}
 %multiplicative subgroup
\newcommand{\zmod}[1]{\Z/{#1}\Z}
\newcommand{\md}[1]{\,(\text{mod }#1)}
%\newcommand{\ks}[1]{K(\sqrt{#1})}
\newcommand{\ksq}[1]{K(\sqrt{#1})/K}
\newcommand{\nksq}[1]{\nm_{K(\sqrt{#1})/K}(K(\sqrt{#1})^{\times})}
\newcommand{\mpp}[0]{\mP/\mfp}

%manifolds
\newcommand{\cvd}[0]{\frac{D}{\partial t}}
\newcommand{\cvs}[0]{\frac{D}{\partial s}}
\newcommand{\np}[1]{\nabla_{\pd{}{#1}}}

%algebraic geometry
%\newcommand{\av}[0]{A^{\vee}}


%arithmetic combinatorics
\newcommand{\Deq}[1]{\Delta^{\times}_{#1}}

%modular forms
\newcommand{\GLAi}[0]{\text{GL}_2(\mathbb A)_{\infty}}

%noise sensitivity part iii essay
\newcommand{\Dict}[0]{\operatorname{\mathsf{Dict}}}
\newcommand{\Maj}[0]{\operatorname{\mathsf{Maj}}}
\newcommand{\MAJ}[0]{\operatorname{\mathsf{Maj}}}
\newcommand{\Parity}[0]{\operatorname{\mathsf{Parity}}}
\newcommand{\Tribes}[0]{\operatorname{\mathsf{Tribes}}}
\newcommand{\Ns}[0]{\operatorname{NS}}
\newcommand{\DT}[0]{\operatorname{\mathsf{DT}}}
\newcommand{\DNF}[0]{\operatorname{\mathsf{DNF}}}
\newcommand{\CNF}[0]{\operatorname{\mathsf{CNF}}}
\newcommand{\Circuit}[0]{\operatorname{\mathsf{Circuit}}}
\newcommand{\Ac}[0]{\mathsf{AC}}
\newcommand{\EB}[0]{\text{EB}}
%comp complexity
%complexity theory
\newcommand{\ACC}[0]{\operatorname{\mathsf{ACC}}}
\newcommand{\BPP}[0]{\mathsf{BPP}}
\newcommand{\BPTIME}[0]{\operatorname{\mathsf{BPTIME}}}
\newcommand{\CLIQUE}[0]{\operatorname{\mathsf{CLIQUE}}}
\newcommand{\EXP}[0]{\mathsf{EXP}}
\newcommand{\NEXP}[0]{\mathsf{NEXP}}
\newcommand{\NC}[0]{\operatorname{\mathsf{NC}}}
\newcommand{\NP}[0]{\operatorname{\mathsf{NP}}}
\newcommand{\NTIME}[0]{\operatorname{\mathsf{NTIME}}}
\newcommand{\msP}[0]{\operatorname{\mathsf{P}}}
\newcommand{\PCP}[0]{\operatorname{\mathsf{PCP}}}
\newcommand{\SAT}[0]{\mathsf{SAT}}
\newcommand{\SUBEXP}[0]{\mathsf{SUBEXP}}
\newcommand{\TIME}[0]{\operatorname{\mathsf{TIME}}}
\newcommand{\zz}{\textcircled{Z}}
%statistics
\newcommand{\hten}[0]{\widehat{\theta_n}}

%EDITING HELP
%blu: key idea or concept. red: unresolved issue/question. 
\newcommand{\blu}[1]{{\color{blue}#1}}
\newcommand{\grn}[1]{{\color{green}#1}}
\newcommand{\redd}[1]{{\color{red}#1}}
\newcommand{\pur}[1]{{\color{purple}#1}}
\newcommand{\oge}[1]{{\color{orange}#1}}
\newcommand{\concept}[1]{#1}
\newcommand{\fixme}[1]{{\color{red}#1}}
\newcommand{\cary}[1]{{\color{purple}#1}}%deprecated
%short for commentary
\newcommand{\llabel}[1]{\label{#1}\text{\fixme{\tiny#1}}}
\newcommand{\nref}[1]{\ref{#1}}
%%%%%%%%%%%
%Use the above when working on the document, so labels will be displayed by their theorems, and you can write reminders to yourself. Switch to the below commands when publishing.
%%%%%%%%%%%
%\newcommand{\fixme}[1]{}
%\newcommand{\concept}[1]{{\color{blue}#1}}
%\newcommand{\llabel}[1]{\label{#1}}
%%%%%%%%%%%

\newcommand{\itag}[1]{\index{#1}[\##1]}
\newcommand{\ilbl}[1]{[#1]\index{#1}}
\newcommand{\iadd}[1]{\index{#1} #1}
\newcommand{\arxiv}[1]{\url{http://www.arxiv.org/abs/#1}}

%markup
\newcommand{\ivocab}[1]{\index{#1}\textbf{#1}}
\newcommand{\vocab}[1]{\textbf{#1}} %also index automatically.
\newcommand{\summq}[1]{\textbf{Summary Question: }#1}
\newcommand{\keypt}[1]{{\it #1}}
\newcommand{\subprob}[1]{\noindent\textbf{#1}\\}
\newcommand{\qatable}[1]{\begin{center}
    \begin{longtable}{ | p{5.5cm} | p{10cm} |}
#1
\end{longtable}
\end{center}}

%Page breaks in equations
\allowdisplaybreaks[2]

%SHA
\DeclareFontFamily{U}{wncy}{}
    \DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
    \DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
    \DeclareMathSymbol{\Sh}{\mathord}{mcy}{"58} 

==> format/packages_colt.tex <==
\usepackage{etex}
%this prevents the "No room for a new \dimen" error that comes from loading too many packages (tikz+xy in particular)

%load geometry first (sets up page)
%\usepackage[top=1.2in, bottom=1.2in, left=1in, right=1in]{geometry}
%\usepackage{fullpage}

%main packages
\usepackage{algorithm}
\usepackage{algorithmicx,algpseudocode}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{array}
\usepackage{bbm}
%\usepackage{asymptote}
\usepackage{cancel}
\usepackage{cmap}
\usepackage{enumerate}
\usepackage{enumitem}%resume lists
%\usepackage{fancyhdr}
%\usepackage{makeidx}
%\usepackage{marvosym}%doesn't work
\usepackage{mathdots}%iddots: dots going northeast
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{hyperref}
%\usepackage{sidecap}
\usepackage{stackrel}
\usepackage{stmaryrd}%\mapsfrom
%\usepackage{tabularx}
%\usepackage{tikz}
%\usepackage{ctable}
\usepackage{titlesec}
\usepackage{titletoc}
\usepackage{url}
\usepackage{verbatim}
\usepackage{wasysym}
\usepackage{wrapfig}
\usepackage{yhmath}
%\usepackage{yhmath}%arcs
\usepackage[all,cmtip]{xy}%Commutative diagrams
%\usepackage[usenames,dvipsnames]{xcolor}%tikz loads xcolor

%load hyperref last
\usepackage{hyperref}
%\usepackage{listings}
%\lstset{
%	basicstyle=\small\ttfamily,
%	keywordstyle=\color{blue},
%	language=python,
%	xleftmargin=16pt,
%}
%this causes an error. No idea why.
% \usepackage[%
% 	firstinits=true,
% 	doi=false,
% 	url=false,
% 	isbn=false,
% 	backend=biber,
% 	style=alphabetic,hyperref]{biblatex}


%\usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric,%
%    decorations.pathreplacing,decorations.pathmorphing,shapes,%
%    matrix,shapes.symbols,shadows,fadings}

%\input xy
%\xyoption{all}

%exclude subsubsections
%\setcounter{tocdepth}{2}



==> format/theorems_std.tex <==
\newtheorem{thm}{Theorem}[section]
\newtheorem*{thm*}{Theorem}
\newtheorem{prb}[thm]{Problem}
\newtheorem*{prb*}{Problem}

\newtheorem{alg}[thm]{Algorithm}
\newtheorem{asm}[thm]{Assumption}
\newtheorem{ax}[thm]{Axiom}
\newtheorem*{ax*}{Axiom}
\newtheorem{clm}[thm]{Claim}
\newtheorem*{clm*}{Claim}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem*{conj*}{Conjecture}
%\newtheorem{cons}{Construction}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{df}[thm]{Definition}
\newtheorem*{df*}{Definition}
\newtheorem{ex}[thm]{Example}
\newtheorem*{ex*}{Example}
\newtheorem{exr}[thm]{Exercise}
\newtheorem{expl}[thm]{Exploration}%prb
\newtheorem{fct}[thm]{Fact}
\newtheorem{lem}[thm]{Lemma}
\newtheorem*{lem*}{Lemma}
\newtheorem{mdl}[thm]{Model}
\newtheorem{pos}[thm]{Postulate}
\newtheorem*{pos*}{Postulate}
%\newtheorem{sprb}{Problem}%numbering for solutions
\newtheorem{pr}[thm]{Proposition}
\newtheorem*{pr*}{Proposition}
\newtheorem{qu}[thm]{Question}
\newtheorem*{qu*}{Question}
\newtheorem{rem}[thm]{Remark}
\newtheorem*{rem*}{Remark}

==> logprojections.tex <==
\section{ONS with a limited number of projections}

The idea is the following. Let $
M=I_d$. Consider the ellipsoid $B(M) = \set{y}{\exists x, \ve{x}_2\le 1, Mx=y} = \set{y}{\ve{(M^\top M)^{-1}M^\top y}_2\le 1}$. Every time we encounter a vector $x_t$ that has large norm with respect to $B(M)$, we add $x_t$ as a row to $M$, and add the constraint $\ve{Ax_t-x_{t+1}}\le 1$. We can show that the volume of $B(M)$ increases by at least a constant factor each time, so this can happen at most logarithmically many times in $T$. Each time it happens, we have to project to a smaller constraint set; this only incurs logarithmically more regret. Moreover, because each $x_t$ can be written as a linear combination of $x_s$'s in $M$ with not-too-large coefficients, $A_tx_t-x_{t+1}$ will never be too large.

(Alternatively, we can choose a large enough $C$ and project to $K_t=\set{A}{\ve{A}_F\le R \text{ and }
\forall s\le t,
\ve{Ax_s-x_{s+1}}_2\le C
}$ each step, and show that the new constraint will not be violated most of the time. However, $C$ depends on the minimal polynomial, so this requires having a bound on the coefficients of the minimal polynomial.)

\begin{algorithm}[h!]
\begin{algorithmic}
\State Input: Description of convex sets $K_0\supeq K_1\supeq \cdots$ (possibly depending on observed $x_t$, $f_t$), $x_1\in K_0\subeq \R^n$, parameters $\ga, \mu>0$.
\State Let $\Si_0=\mu I_n$.
\For{$t=1$ to $T$}
	\State Play $x_t$ and observe cost $f_t(x_t)$.
	\State Update $\Si_t = \Si_{t-1}+\nb_t \nb_t^\top$, where $\nb_t = \nb f_t(x_t)$.
	\State Update $x_{t+1} = \pi_{K_t}^{\Si_t}\pa{x_t - \rc{\ga}\Si_t^{-1}\nb_t}$, where $\pi_{K_t}^{\Si_t}$ denotes projection to $K_t$ in the norm $\ve{x}_{\Si_t} = x^\top \Si_t x$.
\EndFor
\end{algorithmic}
 \caption{Online Newton Step with decreasing sets}
 \label{a:ons-K}
\end{algorithm}

We will use this algorithm with $A_1=O$ and 
\begin{align}
f_t(A) &= \ve{Ax_t-x_{t+1}}^2\\
K_t &= \set{A}{\ve{A}_F\le R \text{ and }
\forall (x,y)\in S_t,
\ve{Ax-y}_2\le 1
}
\end{align}
for $S_t$ containing a subset of pairs $(x_s,x_{s+1})$. We will add $(x_t,x_{t+1})$ to the set only if $x_t$ cannot be written as a linear combination of previous $x_s$'s in $S_t$ with small coefficients. More precisely, we run the following algorithm.

\begin{algorithm}[h!]
\begin{algorithmic}
\State Input: parameters $\ga, \mu>0$.
\State Let $A_1:=O$, $\Si_0:=\mu I_n$, $S_0:=\phi$, $M_0 := I_d$. 
\For{$t=1$ to $T$}
	\State Play $A_t$ and observe cost $f_t(A_t) = \ve{A_tx_t - x_{t+1}}_2^2$.
	\State Update $\Si_t = \Si_{t-1}+\nb_t \nb_t^\top$, where $\nb_t = \nb f_t(x_t)$. \fixme{Compute this, this is in $\R^{d^2\times d^2}$.}
	\If{$\ve{x_t}_{B(M_{t-1})}\ge 2\sqrt d$}
		\State $S_t:=S_{t-1}\cup \{(x_t,x_{t+1})\}$
		\State $M_t:= \coltwo{M_t}{x_t}$
	\Else
		\State $S_t:=S_{t-1}$
		\State $M_t:=M_{t-1}$
	\EndIf
	\State Let $K_t = \set{A}{\ve{A}_F\le R \text{ and }
\forall (x,y)\in S_t,
\ve{Ax-y}_2\le 1}$.
	\State Update $x_{t+1} = \pi_{K_t}^{\Si_t}\pa{A_t - \rc{\ga}\Si_t^{-1}\nb_t}$, where $\pi_{K_t}^{\Si_t}$ denotes projection to $K_t$ in the norm $\ve{A}_{\Si_t} = A^\top \Si_t A$; here $A$ is treated as a vector in $\R^{d^2}$.
\EndFor
\end{algorithmic}
 \caption{Online Newton Step for LDS}
 \label{a:ons-lds}
\end{algorithm}

We start with the general guarantees for Online Newton Step.

\begin{df}
A twice-differentiable $f:\R^n\to \R$ is $\al$-exp-concave at $x$ iff $\nb^2 f(x) \succeq \al \nb f(x) \nb f(x)^\top$.
\end{df}

\begin{thm}
%Suppose $\diam(K_0)\le D$. 
Algorithm~\ref{a:ons-K} with parameters
$\ga \le \al$,  %$\ga = \rc 2 \min\{\rc{4GD},\al\}$, 
$\mu = \rc{\ga^2D^2}$ and $T>4$ guarantees
\begin{align*}
R_T &\le %5\pa{\rc \al + GD}n \ln T.
\rc{2\ga} \pa{n\ln (TG^2D^2\ga+1)}
+
\sumo tT \ve{\pi_{K_t}^{\Si_t}(x_t-\rc{\ga}\Si_t^{-1}\nb_t) - 
\pi_{K_{t-1}}^{\Si_t}(x_t-\rc{\ga}\Si_t^{-1}\nb_t)}_2^2\\
&\le 
\rc{2\ga} \pa{n\ln (TG^2D^2\ga+1)} +
D^2 \#\set{1\le t\le T}{K_t\ne K_{t-1}}.
\end{align*}
Here, $\al$ is such that each $f_t$ is $\al$-exp-concave at $x_t$, $\ve{\nb_t}\le G$, the diameter of $K_0$ is at most $D$. 
\end{thm}
\begin{proof}
See Theorem 4.3 in [OCO, Hazan]. The only changes are that we keep $\ga\le \al$ and that we are projecting to a shrinking sequence of sets, $K_{t}$ at step $t$, instead of a fixed $K_0$, and so incur the extra sum. \fixme{Actually I don't think you incur the extra term at all so the previous proof works!}
\end{proof}


\begin{lem}
Suppose that $x_t = \sum_{(x,y)\in S_{t-1}} a_xx$ with $\ve{x_t}_{B(M_{t-1})}\le L$. Then for any $A\in K_{t-1}$,
\begin{align}
\ve{Ax_t-x_{t+1}}_2
&\le 2L \sqrt{|S_{t-1}|+R^2}+1.
\end{align}
\end{lem}
\begin{proof}
The bound $\ve{x_t}_{B(M_{t-1})}\le L$ means that there exist coefficients $a_x$  such that  
\begin{align}
x_t &= \sum_{(x,y)\in S_{t-1}} a_x x
 + \sumo id a_i e_i
\end{align}
with $\sum_{(x,y)\in S_{t-1}}  a_x^2 + \sumo id a_i^2=L$. 
For $(x,y)\in S_{t-1}$ and $A\in K_{t-1}$, we have $\ve{Ax-y}_2\le1$ by definition of $K_{t-1}$; moreover by assumption, $\ve{A^*x-y}_2\le 1$. Thus, $\ve{Ax-A^*x}_2\le 1$.
Then by Cauchy-Schwarz,
\begin{align}
Ax_t - A^* x_t &=
\sum_{(x,y)\in S_{t-1}} \al_x (Ax-A^*x) + \sumo id a_i (Ae_i-A^*e_i)\\
\ve{Ax_t - A^*x_t}_2 &\le 
2\sum_{(x,y)\in S_{t-1}}|\al_x| + 
\sqrt{\sumo id a_i^2}\cdot 2R\\
&\le 2\sqrt{\sum_{(x,y)\in S_{t-1}} \al_x^2} \sqrt{|S_{t-1}|} + 2 \sqrt{\sumo id a_i^2}\cdot R\\
&\le 2L \sqrt{|S_{t-1}| + R^2}
\end{align}
\end{proof}


==> main.tex <==
% % *LICENSE AGREEMENT FORM* The hyperlink for the permissions form in previous email was missing. Please fill in the form at http://proceedings.mlr.press/pmlr-license-agreement.pdf

% % *BIBTEX FILE* for the tag "pages" - please use {1--<lastpage number>}

% % For authors who choose the Extended Abstract version. Please note the following information (which are in addition to the instructions for the full paper): 

% % *EXTENDED ABSTRACT* An "extended abstract" should be at least one page long (but otherwise subject to the same limits as regular papers), using the same LaTeX format as regular papers. Please put the full version on arXiv with a footnote "Accepted for presentation at the Conference on Learning Theory (COLT) 2019" on the front page. Include the following footnote on the front page: "Extended abstract. Full version appears as [arXiv reference, v#]", where v# is the version number of the full version.

% %\documentclass[11pt]{article}  
% \documentclass[final]{colt2020}

% \input{format/packages_colt}
% %\input{theorems_std.tex}
% \input{format/defs_colt}
% %\input{macros.tex}
% %\newcommand{\citep}[1]{\cite{#1}}
% %\usepackage[linesnumbered,ruled]{algorithm2e}
% %\usepackage{algorithm}
% %\usepackage{algorithmic}
% \usepackage{times}

% \usepackage{etoolbox}

% %can't load amsthm...
% \newcommand{\qedhere}[0]{}
% %\addbibresource{bib.bib}

% \renewcommand{\llabel}[1]{\label{#1}}
% % \renewcommand{\hl}[1]{}
% % \renewcommand{\ks}[1]{}
% % \renewcommand{\ug}[1]{}

% \begin{document}

% \title{No-Regret Prediction in Marginally Stable Systems}


% \coltauthor{%
%  \Name{Udaya Ghai} \Email{ughai@cs.princeton.edu}\\
%  \addr Princeton University
%  \AND
%  \Name{Holden Lee} \Email{holee@math.duke.edu}\\
%  \addr Duke University
%   \AND
%  \Name{Karan Singh} \Email{karans@princeton.edu}\\
%  \addr Princeton University
%   \AND
%  \Name{Cyril Zhang} \Email{cyril.zhang@princeton.edu}\\
%  \addr Princeton University
%   \AND
%  \Name{Yi Zhang} \Email{y.zhang@princeton.edu}\\
%  \addr Princeton University
% }

% % \author{
% % Udaya Ghai, Holden Lee, Karan Singh, Cyril Zhang, Yi Zhang %\\
% %   %Department of Computer Science\\
% %   %Princeton University\\
% %   %Princeton, NJ 08544 \\
% % %Holden Lee\thanks{Princeton University, Mathematics Department \texttt{holdenl@math.princeton.edu}}, Cyril Zhang\thanks{Princeton University, Computer Science Department \texttt{cyril.zhang@cs.princeton.edu}}
% % }
% %add names



% \date{\today}
% \maketitle
% %\tableofcontents

% \input{main/0-abstract}

% \begin{keywords}%
%   Dynamical systems, marginally stable systems, online least squares.
% \end{keywords}

% %\hl{NOTE: COLT automatically loads algorithm2e, which clashes with algorithmcx, the current package loaded by the paper. I commented out algorithm2e in jmlr.cls. We need to convert algorithmcx syntax to algorithm2e in the final version. See \url{https://tex.stackexchange.com/questions/229355/algorithm-algorithmic-algorithmicx-algorithm2e-algpseudocode-confused}}

% \input{main/1-intro}
% \input{main/2-related}
% \input{main/3-results}
% \input{main/4-proof_sketch}
% \input{main/conclusion}
% \bibliography{bib}
% \appendix 
% \input{main/5-ols}
% \input{main/6-body}
% \input{main/ols-regret}
% \input{main/php-approach}
% \input{main/openq}

% %\printbibliography
% %\appendix


% \end{document}



==> old.tex <==
\appendix

\subsection{Marginal stability and phase separation}
The hardest regime to analyze is when the dynamics are \emph{marginally stable}; that is, when the state dependences do not grow or shrink exponentially with time. 

Let $\theta_i \in [0, 2\pi)$ denote the phase of $\lambda_i$, so that $\lambda_i = |\lambda_i| e^{2 \pi i \theta_i}$.

For any $i \neq j$, we assume $|\theta_i - \theta_j| \geq \gamma$.

\section{Main theorem}
\label{sec:results}
\begin{theorem}
Algorithm~\ref{alg:least-squares} produces a sequence of estimates $(\hat x_1, \ldots, \hat x_t)$ which satisfy the regret bound
\[ \sum_{t=1}^T \norm{\hat x_t - x_t}^2 \leq \sum_{t=1}^T \norm{\eps_t}^2 + O(\log T). \]
\end{theorem}

Possibly include: Important independent lemmas. Corollaries. Alternate forms.

\subsection{Discussion}
\label{subsec:results-discussion}
Justify exponential dependence on dimension: other papers, example systems. Lower bound possible?

\section{Proofs}
\label{sec:proofs}

\subsection{Noiseless case}
\label{subsec:proofs-noiseless}

In this section, we consider a simplified setting where the noise $\varepsilon_t$ is zero at every time step.

The algorithm is simply Follow-the-Leader:
\begin{align*}
    A_t = \arg\min_{A} \sum_{s=1}^{t-1} \|A_s x_s - x_{s+1}\|_2^2 = A^*\sum_{s=1}^{t-1} (x_s x_s^\top) (\sum_{s=1}^{t-1} x_s x_s^\top)^{-1} = A^* P_U
\end{align*}
%where $\-1$ denotes the pseudo-inverse and $P_U$ is the projection matrix onto the column space of $\sum_{s=1}^{t-1} x_s x_s^\top$.

Note that $A_t$ acts perfectly the same as the ground-truth $A^*$ meaning that if $x_t$ always stays in the span of $\{x_1, x_2,\ldots, x_{t-1}\}$, then no regret would be incurred. We show in the following this in fact happens at any time step $t>d$.

\begin{theorem}
\label{thm:structural}
For any $t>d$ and any $x\in\R^d$ and any $A\in\R^{d\times d}$, $A^tx\in \spn\{Ax, A^2x, \ldots, A^dx\}$.
\end{theorem}

\begin{proof}
Consider the (possibly complex) eigen-decomposition of $A=U\Lambda U^{-1}$ where $\Lambda=\text{diag}(\lambda_1, \lambda_2, \ldots, \lambda_d)$, the condition that $A^t$ in the span is equivalent to there exists a vector $\alpha\in\mathbb{R}^d$ such that
\begin{align*}
\begin{bmatrix}
\lambda_1^t\\
\lambda_2^t\\
\vdots\\
\lambda_d^t
\end{bmatrix} = \begin{bmatrix}
\lambda_1 & \lambda_1^2 & \ldots & \lambda_1^d\\
\lambda_2 & \lambda_2^2 & \ldots & \lambda_2^d\\
\vdots & \vdots & \ddots & \vdots \\
\lambda_d & \lambda_d^2 & \ldots & \lambda_d^d\\
\end{bmatrix} \begin{bmatrix}
\alpha_1\\
\alpha_2\\
\vdots\\
\alpha_d
\end{bmatrix}
\end{align*}.

This is true by observing that we can assume all $\lambda$'s are non-zero without loss of generality and then $\begin{bmatrix}
\lambda_1 & \lambda_1^2 & \ldots & \lambda_1^d\\
\lambda_2 & \lambda_2^2 & \ldots & \lambda_2^d\\
\vdots & \vdots & \ddots & \vdots \\
\lambda_d & \lambda_d^2 & \ldots & \lambda_d^d\\
\end{bmatrix}$ is full-rank because its determinant is $\prod_{i\not=j}(\lambda_i - \lambda_j)$
\end{proof}
\yz{One can also use Cayley-Hamilton.}
Theorem~\ref{thm:structural} suggests that regret is only incurred in the first $d$ rounds prediction under the noise-free assumption. Since the $l_t= O(d^2)$ for any $t\leq d$, the total amount of regret should be $R_T\leq \text{poly}(d)$ which is independent of $T$.
\ug{Since there is no noise, don't we have $l_t \leq 4$ and so regret is $O(d)$?  Or are we trying to handle
case where matrix can explode as well?}



\subsection{Observable noise}
\label{subsec:proofs-observable}

The algorithm is simply Follow-the-Leader:
\begin{align*}
    A_t = \arg\min_{A} \sum_{s=1}^{t-1} \|A_s x_s + \varepsilon_s - x_{s+1}\|_2^2 = A^*\sum_{s=1}^{t-1} (x_s x_s^\top) (\sum_{s=1}^{t-1} x_s x_s^\top)^{-1} = A^* P_U
\end{align*}
where $-1$ denotes the pseudo-inverse and $P$ is the projection matrix onto the column space of $\sum_{s=1}^{t-1} x_s x_s^\top$. Note that $A_t$ acts perfectly identical to the ground-truth $A^*$ in the subspace and is zero outside.

\begin{theorem}
$x_t - u\in\spn\{x_{t-d-1}, x_{t-d},\ldots,x_{t-1}\}$ for some $u\in\mathbb{R}^d$ with $\|u\|_2 = C_{d}$ where $C_d$ only depends on $A^*$.
\end{theorem}

\begin{proof}
By theorem~\ref{thm:structural}, we have $A^{d+1} x_{t-d-1} = \sum_{i=1}^{d} \alpha_i A^i x_{t-d-1}$. We denote the size of the coefficient $\|\alpha\|_1$ by $C$ which is determined by $A^*$. Note that for any $1\leq i\leq d$,
\begin{align*}
    x_{t-d-1+i} = A^i x_{t-d-1} + \sum_{\tau=1}^i A^{i-\tau}\varepsilon_{t-d-1+\tau} = A^i x_{t-d-1} + u_i
\end{align*}
and $\|u_i\|_2=O(\text{poly}(d))$. Now, we write $x_t$ as
\begin{align*}
    x_t &= A^{d+1} x_{t-d-1} + \sum_{\tau=1}^{d+1} A^{d+1-\tau}\varepsilon_{t-d-1+\tau} = A^{d+1} x_{t-d-1} + u_{d+1}\\
        &= u_{d+1} + \sum_{i=1}^{d+1} \alpha_i A^i x_{t-d-1} = u_{d+1} + \sum_{i=1}^{d+1} \alpha_i (x_{t-d-1+i} - u_i)\\
        &= u_{d+1} - \sum_{i=1}^{d+1} \alpha_i u_i + \sum_{i=1}^{d+1} \alpha_i x_{t-d-1+i}
\end{align*}
Thus $x_t - u$ lies in $\spn\{x_{t-d-1}, x_{t-d},\ldots,x_{t-1}\}$ with $u = -u_{d+1} + \sum_{i=1}^{d+1} \alpha_i u_i$ whose $\ell_2$ norm is independent of $T$ but rather depends on dimension $d$ as well as the size of coefficients of the characteristic polynomial of $A^*$ which might be exponential in $d$ in the worst case.
\end{proof}

As a direct corollary of the above theorem, we show a sublinear regret bound of the FTL algorithm.
\begin{corollary}
In the observable noise setting, FTRL achieves the regret $R_T\leq C_d\log T$
\end{corollary}
\begin{proof}
\begin{align*}
    \|A_tx_t + \varepsilon_t - x_{t+1}\|_2^2 = \|(A_t - A^*)x_t\|_2^2  = \|(A_t - A^*) u \|_2^2\leq \|A^* \|_2^2 \| I - P\|_2^2 \|v\|_2^2 \leq \|A\|_2^2 \|v\|_2^2
\end{align*}
since $A_t$ and $A^*$ behave identically in $\spn\{x_{t-d-1}, x_{t-d},\ldots,x_{t-1}\}$.
\end{proof}

\subsection{Unobservable noise}
\label{subsec:proofs-full}

First, let us introduce some notation for readability. Upon writing $x_t$ in the eigenbasis of $A^*$, the coefficients are given by $V^{-1} x_t$. For any $i \in 1, \ldots, d$, we will denote by $(V^{-1} x_t)_i$ the $i$-th coordinate of this expansion $V^{-1} x_t$. Similarly, $(V^{-1} \eps_t)_i$ will denote the $i$-th coordinate of $V^{-1} \eps_t$.


The algorithm is still Follow-the-Leader:
\begin{align*}
    A_t = \arg\min_{A} \sum_{s=1}^{t-1} \|A_s x_s - x_{s+1}\|_2^2 = (A^*\sum_{s=1}^{t-1} (x_s x_s^\top) + \sum_{s=1}^{t-1} (\varepsilon_s x_s^\top)) (\sum_{s=1}^{t-1} x_s x_s^\top)^{-1} = A^* P_U + \hat{A_t}
\end{align*}

where $\hat{A}=(\sum_{s=1}^{t-1} \varepsilon_s x_s^\top)(\sum_{s=1}^{t-1} x_s x_s^\top)^{-1}$


\begin{lemma}
\label{lemma:circle}
For any complex numbers $\lambda_1, \lambda_2 \in \mathbb{C}$ and any $t\in\mathbb{Z}^+$, if $\lambda_1 \overline{\lambda_2} = a e^{i\theta}$ where $0 \leq a\leq 1+\frac{C}{t+1}$ for some constant $ 0 < C < t$ and $| \theta | > 0$,   then $\left| \sum_{s=1}^{t} (\lambda_1 \overline{\lambda_2})^s \right| \leq  O\left(e^C / \sin(\theta) \right)$.
\end{lemma}

\begin{proof}
\begin{align*}
    \left| \sum_{s=1}^{t} (\lambda_1 \overline{\lambda_2})^s \right| &= \left| \sum_{s=1}^t \left( ae^{i\theta} \right)^t \right| = \left| \frac{1 - a^{t+1} e^{i (t+1)\theta}}{1 - a e^{i\theta}} \right|  \\
    &\leq \left| \frac{1}{1 - a e^{i\theta}}  \right| +  a^{t+1} \left| \frac{e^{i(t+1)\theta}}{1 - a e^{i\theta}}  \right| \leq (1 + e^C) \left| \frac{1}{1 - a e^{i\theta}}  \right| \\
    &\leq \frac{1+e^C}{\sqrt{(1-a)^2 + 2a (1-\cos(\theta)} ) } \leq \frac{1 + e^C}{\sin(\theta)}
\end{align*}
\end{proof}

Writing $G = \sum_s^{t-1} V^{-1}x_s x_s^\top V^{-\top} $, $\beta = V^{-1} x_{t}$, and $\mathcal{E} = \sum_{s=1}^{t-1}V^{-1} \epsilon_s x_s^{\top} V^{-\top} $, we show in the following that in order to bound the residual error $\| \hat{A}_t x_t \|_2$, it suffices to bound $\| \mathcal{E} G^{-1} \beta \|_2 $ under the assumption $\kappa = O(1)$.
\begin{align*}
    \hat{A}_t x_t  &=   (\sum_{s=1}^{t-1} \varepsilon_s x_s^\top)(\sum_{s=1}^{t-1} x_s x_s^\top)^{-1} x_t \\
    &= V \left( \sum_{s=1}^{t-1} V^{-1} \epsilon_s x_s^{\top}  V^{-\top} \right)  V^\top \left[ V \left( \sum_s^{t-1} V^{-1}x_s x_s^\top  V^{-\top}  \right) V^\top \right]^{-1} V \left(V^{-1} x_t \right) \\ 
    &= V \left( \sum_{s=1}^{t-1} V^{-1} \epsilon_s x_s^{\top}  V^{-\top} \right)  \left( \sum_s^{t-1} V^{-1}x_s x_s^\top  V^{-\top}  \right)^{-1} \left(V^{-1} x_t \right) \\
    &= V \mathcal{E} G^{-1} \beta \\
\end{align*}

\begin{lemma}
\begin{align*}
    \left\lVert \hat{A}_t x_t \right\rVert_2^2 \leq ~t~x_t^\top \left(\mu I + \sum_{s=1}^{t-1} x_s x_s^\top \right)^{-1} x_t = ~t~ \beta^\top \left(\mu I + G \right)^{-1} \beta
\end{align*}
\end{lemma}

\begin{proof}

\end{proof}

\begin{align*}
\left\lVert \hat{A}_t x_t \right\rVert_2^2 = \left\lVert x_t^\top (\sum_{s=1}^{t-1} x_s x_s^\top)^{-1} (\sum_{s=1}^{t-1} x_s \varepsilon_s^\top) (\sum_{s=1}^{t-1}  \varepsilon_s x_s^\top)(\sum_{s=1}^{t-1} x_s x_s^\top)^{-1} x_t \right\rVert_2^2     
\end{align*}

Now we partition the coordinates of $\beta$ into two groups i.e. $ \beta_1$ and $\beta_2$ by setting a threshold of $L t^{4/9}$ and rearrange the rows of $\mathcal{E}$ accordingly into $\mathcal{E}_1$ and $\mathcal{E}_2$ so that every entry in $\beta_1$ and $\mathcal{E}_1$ are larger than $Lt^{4/9}$ in magnitude and the rest are smaller.
\begin{align*}
      \hat{A}_t x_t = V \begin{bmatrix}
      \mathcal{E}_1 & \mathcal{E}_2 \\
      \end{bmatrix} (\mu I + G)^{-1} \begin{bmatrix}
      \beta_1\\
      \\
      \beta_2
      \end{bmatrix} \\
\end{align*}

The next lemma shows we can safely ignore the small subspaces $\beta_2$ and $\mathcal{E}_2$ at the cost of enlarging the loss by $O(L^2 t^{8/9})$ \emph{additively}.
\begin{lemma}
If $\mu$ is set to be $L^2 t^{8/9}$,
\begin{align*}
      \| \hat{A}_t x_t \|_2 \leq \kappa \left\lVert \begin{bmatrix}
      \mathcal{E}_1 & 0\\
      \end{bmatrix} (\mu I + G)^{-1} \begin{bmatrix}
      \beta_1\\
      \\
      0
      \end{bmatrix} \right\rVert_2 + ???\\
\end{align*}
\end{lemma}

\begin{proof}
\begin{align*}
     \left\lVert \begin{bmatrix}
      \mathcal{E}_1 & \mathcal{E}_2\\
      \end{bmatrix} (\mu I + G)^{-1} \begin{bmatrix}
      \beta_1\\
      \\
      \beta_2
      \end{bmatrix} - \begin{bmatrix}
      \mathcal{E}_1 0\\
      \end{bmatrix} (\mu I + G)^{-1} \begin{bmatrix}
      \beta_1\\
      \\
      0
      \end{bmatrix} \right\rVert_2 \\
      \leq  \underbrace{\left\lVert \begin{bmatrix}
      \mathcal{E}_1 & \mathcal{E}_2\\
      \end{bmatrix} (\mu I + G)^{-1} \right\rVert_2 \left\lVert
      \begin{bmatrix}
      0\\
      \\
      \beta_2
      \end{bmatrix} \right\rVert_2}_{\Delta_1}
      + \underbrace{\left\lVert \begin{bmatrix}
      0 & \mathcal{E}_2\\
      \end{bmatrix} (\mu I + G)^{-1} \right\rVert_2 \left\lVert
      \begin{bmatrix}
      \beta_1\\
      \\
      0
      \end{bmatrix} \right\rVert_2}_{\Delta_2}
\end{align*}
$\Delta_1$ and $\Delta_2$ can be bounded separately as follows.
\begin{align*}
    \Delta_1 & \leq \left\lVert \begin{bmatrix}
      \mathcal{E}_1 & \mathcal{E}_2\\
      \end{bmatrix} (\mu I + G)^{-1} \right\rVert_2 \left\lVert
      \begin{bmatrix}
      0\\
      \\
      \beta_2
      \end{bmatrix} \right\rVert_2 \\
      & \leq \left( \left\lVert \begin{bmatrix}
      \mathcal{E}_1 & 0\\
      \end{bmatrix} (\mu I + G)^{-1} \right\rVert_2 + \left\lVert \begin{bmatrix}
      0 & \mathcal{E}_2\\
      \end{bmatrix} (\mu I + G)^{-1} \right\rVert_2 \right)
      \left\lVert
      \begin{bmatrix}
      0\\
      \\
      \beta_2
      \end{bmatrix} \right\rVert_2 \\
      & \leq \left( \left\lVert \begin{bmatrix}
      \mathcal{E}_1 & 0\\
      \end{bmatrix} G^{-1} \right\rVert_2 + \left\lVert \begin{bmatrix}
      0 & \mu^{-1}\mathcal{E}_2\\
      \end{bmatrix} \right\rVert_2 \right)
      \left\lVert
      \begin{bmatrix}
      0\\
      \\
      \beta_2
      \end{bmatrix} \right\rVert_2 \\
\end{align*}

The entries of $\mu^{-1}\mathcal{E}_2$ are $O(1)$ since the entries of $\mathcal{E}_2$ are $O(\sum_{s=1}^{t-1} f_i(s))$ while $$.$$
\end{proof}




For convenience of presentation, we introduce a few new notations. We denote by $f_m(s)$ the value of $\left| \left(V^{-1} x_s \right)_m \right|$. Under this notation, we have $G_{m,m} = \sum_{s=1}^{t-1} f_m(s)^2$ and $G_{m,n} = C_3\left(O(t) + \sum_{s=1}^{t-1} f_m(s) + f_n(s) \right)$.

\begin{lemma}
\label{lemma:lipschitz}
For any $1\leq m\leq d$ such that $|\lambda_m|\leq 1 + O(1/t)$, $f_m(t)$ is $O(1)-$Lipschitz w.r.t. $t$. Specifically, if $|\lambda_m|\leq 1 + C/t$, then we have for any $0\leq s < t$
\begin{align*}
    \left| f_m(s) - f_m(s-1) \right| = \kappa e^C
\end{align*}
\end{lemma}

\begin{proof}
\begin{align*}
   \left| f_m(t) - f_m(t-1) \right| &= \left| \left| \left( V^{-1} x_t \right)_m \right| - \left| \left( V^{-1} x_{t-1} \right)_m  \right| \right| \\
   &= \left| \left| \left( V^{-1} \epsilon_t \right)_m \right| +  (1-|\lambda_m|) \left| \left( V^{-1} x_{t-1} \right)_m  \right| \right| \\
   & \leq \left| \left( V^{-1} \epsilon_t \right)_m \right| +  |1-|\lambda_m|| \sum_{i=0}^{t-2} |\lambda_m|^i \left| \left( V^{-1} \epsilon_{t-1-i} \right)_m  \right|  \\
   & \leq \kappa + \kappa \left| 1 - |\lambda_m|^{t-1}\right|\\
   & \leq \kappa e^C
\end{align*}
The inequality is tight when $|\lambda_m| =1 + C/t$.
\end{proof}

\begin{lemma}
Using the notation $f_m(s)=\left| \left(V^{-1} x_s \right)_m \right|$, we have the following 
\begin{align*} 
G_{m,m} & = \sum_{s=1}^{t-1} f_m(s)^2\\
\left| G_{m,n} \right| & = O(t) + O\left(\sum_{s=1}^{t-1} f_m(s) + f_n(s)\right)
\end{align*}
for any $m\not=n$ where $O(\cdot)$ hides constants independent of $t$.
\end{lemma}
\begin{proof}

The diagonal terms of $G$ take simple forms,
\begin{align*}
    G_{m,m} = \left( \sum_s^{t-1} V^{-1}x_s x_s^\top V^{-\top} \right)_{m,m} = \sum_{s=1}^{t-1} \left| \left( V^{-1} x_s \right)_m \right|^2
\end{align*}

while the off-diagonal requires more attention,

\begin{align*}
    &G_{m,n}^t = \left( \sum_{s=1}^{t-1} V^{-1}x_s x_s^\top V^{-\top} \right)_{m,n} = \sum_{s=1}^{t-1} \left( V^{-1} x_s \right)_m  \left( \overline{ V^{-1} x_s} \right)_n = \sum_{s=1}^{t-1} \left( V^{-1} \sum_{i=1}^{s} A^{s-i} \epsilon_i \right)_m \left(\overline{ V^{-1} \sum_{i=1}^{s} A^{s-i} \epsilon_i} \right)_n \\
    &= \sum_{s=1}^{t-1} \left( \sum_{i=1}^{s} \Lambda^{s-i} V^{-1}\epsilon_i \right)_m \left( \overline{ \sum_{i=1}^{s} \Lambda^{s-i} V^{-1}\epsilon_i} \right)_n  = \sum_{s=1}^{t-1} \sum_{i,j=1}^{s} \lambda_m^{s-i} \overline{\lambda_n}^{s-j} \left(V^{-1}\epsilon_i \right)_m \left(\overline{V^{-1}\epsilon_j} \right)_n \\
    &= \sum_{i < j}^{t-1} \lambda_m^{j-i} \left(V^{-1}\epsilon_i \right)_m  \left(\overline{V^{-1}\epsilon_j} \right)_n \left[ \sum_{s=j}^{t-1} (\lambda_m \overline{\lambda_n} )^{s-j}  \right] + \sum_{i > j}^{t-1}  \left(V^{-1}\epsilon_i \right)_m \left(\overline{V^{-1}\epsilon_j} \right)_n \overline{\lambda_n}^{i-j} \left[ \sum_{s=i}^{t-1} (\lambda_m \overline{\lambda_n})^{s-i} \right] \\
    &+ \sum_{i=1}^{t-1} \left(V^{-1}\epsilon_i \right)_m  \left(\overline{V^{-1}\epsilon_j} \right)_n \left[ \sum_{s=j}^{t-1} (\lambda_m \overline{\lambda_n} )^{s-j}  \right] \\
    &= \sum_{j=1}^{t-1} \left[ \sum_{i=1}^{j} \lambda_m^{j-i} \left(V^{-1}\epsilon_i \right)_m \right]  \left(\overline{V^{-1}\epsilon_j} \right)_n \left[ \sum_{s=j}^{t-1} (\lambda_m \overline{\lambda_n} )^{s-j}  \right] + \sum_{i = 1}^{t-1}  \left(V^{-1} \epsilon_i \right)_m \left[ \sum_{j=1}^{i-1} \left(\overline{V^{-1}\epsilon_j} \right)_n \overline{\lambda_n}^{i-j} \right] \left[ \sum_{s=i}^{t-1} (\lambda_m \overline{\lambda_n})^{s-i} \right] \\
    &+  \sum_{i=1}^{t-1} \left(V^{-1}\epsilon_i \right)_m  \left(\overline{V^{-1}\epsilon_j} \right)_n \left[ \sum_{s=j}^{t-1} (\lambda_m \overline{\lambda_n} )^{s-j}  \right]\\
    &= \sum_{i=1}^{t-1} \left[ \left(V^{-1} x_i \right)_m  \left(\overline{V^{-1} \epsilon_i} \right)_n + \left(V^{-1} \epsilon_i \right)_m  \left(\overline{V^{-1} x_i} \right)_n + \left(V^{-1}\epsilon_i \right)_m  \left(\overline{V^{-1}\epsilon_j}\right)_n \right] \left[ \sum_{s=i}^{t-1} (\lambda_m \overline{\lambda_n})^{s-i} \right] 
\end{align*}

Now we utilize the Lemma~\ref{lemma:circle} to bound the off-diagonal entries of $G$ as follows
\begin{align}
    \left| G_{m,n} \right| &\leq \sum_{i=1}^{t-1} \left[ \left| \left(V^{-1} x_i \right)_m  \left(\overline{V^{-1} \epsilon_i} \right)_n \right| 
    + \left| \left(V^{-1} \epsilon_i \right)_m \left(\overline{V^{-1} x_{i-1}} \right)_n \right| + \left| \left(V^{-1} \epsilon_i \right)_m  \left(\overline{V^{-1} \epsilon_i} \right)_n \right| \right] 
    \left[ \sum_{s=i}^{t-1} (\lambda_m \overline{\lambda_n})^{s-i} \right] \nonumber \\
    & \leq \frac{2e^C}{\sin(\theta_{m,n})} \sum_{i=1}^{t-1}  \left| \left(V^{-1} x_i \right)_m  \left(\overline{V^{-1} \epsilon_i} \right)_n \right| 
    + \left| \left(V^{-1} \epsilon_i \right)_m \left(\overline{V^{-1} x_i} \right)_n \right| 
    + \left| \left(V^{-1} \epsilon_i \right)_m  \left(\overline{V^{-1} \epsilon_i}\right)_n \right| \label{ineq:crossterm_bound} \\
    & \leq \frac{2 \kappa ~e^C}{\sin(\theta_{m,n})} \sum_{i=1}^{t-1}  \left| \left(V^{-1} x_i \right)_m \right| 
    + \left| \left(\overline{V^{-1} x_i} \right)_n \right|    + \kappa \nonumber \\
    & \leq C_3 \left( t\kappa + \sum_{i=1}^{t-1}  \left| \left(V^{-1} x_i \right)_m \right| 
    + \left| \left(\overline{V^{-1} x_i} \right)_n \right| \right) \nonumber
\end{align}
where $C_3$ is a shorthand symbol for $\max_{m,n}\frac{2 + 2\kappa e^C}{\sin(\theta_{m,n})}$.



\end{proof}

Now we inspect relative magnitude of the diagonal terms $G_{m,m}$ versus off-diagonal terms $G_{m,n}$, in order to show the diagonal dominance of $G$. To gain some intuition, let us consider an easy case where $ f_m(t) = \Theta(t)$ (i.e. grows linearly with time $t$). The Lipschitzness of $f_m(s)$  (Lemma~\ref{lemma:lipschitz}) asserts that $f_m(t)$ must have stayed as large las $\Theta(t)$ for $\Theta(t)$ time steps. Then a few elementary calculations show that $G_{m,m}=\Theta(t^3)$ while $G_{m,n}$ is only $\Theta(t^2)$.

However, the same statement is not true if $f_m(t)$ doesn't grow at all. In the following, we prove as long as $f_m(t)=\Omega(t^{4/9})$, the the diagonal entries still dominate the off-diagonal ones.

\begin{lemma}
\label{lemma:digonal-dominance}
If for all $1\leq m\leq d$, $f_m(t) \geq \Omega(t^{4/9})L$ and $t>\Omega\left(d! \kappa^2 C_3^2 / L^4 \right)^9$, then we have
\begin{align*}
 \left| G_{n,m} \right| = \left| G_{m,n} \right| \leq \frac{1}{\sqrt{2d!}}\sqrt{G_{m,m} G_{n,n}}
\end{align*}
for any $m\not=n$.
\end{lemma}

\begin{proof}


To compare $G_{m,m}$ to $G_{m,n}$, let us examine them term by term. $f_m(s)^2 \leq C_3 f_m(s)$ is possible only if $f_m(s)\leq C_3$. This can only be true for $0\leq s\leq t - t^{5/12}$, since $f_{m}(s)$ needs to climb up to $(t^{5/12} + C_3)L$ in the end, with stepsize at most $L$. Therefore
\begin{align*}
& \sum_{s=1}^{t-1}f_m(s)^2 - (d!)^{1/2} C_3 \left( t \frac{\kappa}{2} + \sum_{s=1}^{t-1}f_m(s) \right) \\
&= - (d!)^{1/2} C_3 \frac{\kappa}{2} t + \sum_{s=1}^{\left \lceil {t - t^{5/12} } \right \rceil} f_m(s)^2 - d!C_3 f_m(s) + \sum_{s=\left \lceil {t - t^{5/12} } \right \rceil+1}^{t-1} f_m(s)^2 - (d!)^{1/2} C_3 f_m(s) \\
& = - (d!)^{1/2} C_3 \left( \frac{\kappa}{2} + C_3 \right) t - (d!)^{1/2} C_3 t^{5/6} + \frac{1}{3} t^{5/4} \\
& \geq  - (d!)^{1/2} C_3 \left( \frac{\kappa}{2} + C_3 + 1 \right) t + \frac{1}{3} t^{5/4} \\
& \geq 0
\end{align*}
where the last step uses the assumption $t > 81 \left(  (d!)^{1/2} C_3 \left( \frac{\kappa}{2} + C_3 + 1 \right) \right)^4 $. The above inequality implies
\begin{align}
  \sum_{s=1}^{t-1}f_m(s)^2  \geq (d!)^{1/2} C_3 \left( t \frac{\kappa}{2} + \sum_{s=1}^{t-1}f_m(s) \right)
\end{align}
and therefore
\begin{align}
\label{ineq:diagonal}
  \left(\sum_{s=1}^{t-1}f_m(s)^2 \right)  \left( \sum_{s=1}^{t-1}f_n(s)^2 \right)  \geq d! C_3^2 \left( t \frac{\kappa}{2} + \sum_{s=1}^{t-1}f_m(s) \right) \left( t \frac{\kappa}{2} + \sum_{s=1}^{t-1}f_n(s) \right)
\end{align}

\begin{align*}
    & \left( \sum_{s=1}^{t-1}f_m(s)^2 \right) \left( \sum_{s=1}^{t-1}f_n(s)^2 \right) \geq L^2\left( t^{4/9} \right)^3 \left( \sum_{s=1}^{t-1}f_n(s)^2 \right) \geq L^2 t^{1/3}\left( \sum_{s=1}^{t-1}f_n(s) \right)^2\\
    &\geq L^2 t^{1/3} \left(\frac{\sum_{s=1}^{t-1}f_n(s)}{\kappa t/2 + \sum_{s=1}^{t-1}f_n(s)} \right)^2 \left(\kappa t/2 + \sum_{s=1}^{t-1}f_n(s) \right)^2 \\
    & \geq L^2 t^{1/3} \left(\frac{Lt^{8/9}}{\kappa t/2 + Lt^{8/9}}\right)^2 \left(\kappa t/2 + \sum_{s=1}^{t-1}f_n(s) \right)^2\\
    & \geq \frac{L^4}{\kappa^2} t^{1/3 - 2/9}\left(\kappa t/2 + \sum_{s=1}^{t-1}f_n(s) \right)^2 \\
    & \geq \frac{L^4}{\kappa^2} t^{1/9} \left( \kappa t/2 +  \sum_{s=1}^{t-1}f_m(s) \right)^2
\end{align*}
where in the middle we used that for any vector $a\in\R^{t}$, $\sqrt{t}\|a\|_2\geq \|a\|_1$. In the same vein, we can show
\begin{align*}
    & \left( \sum_{s=1}^{t-1}f_m(s)^2 \right) \left( \sum_{s=1}^{t-1}f_n(s)^2 \right) \geq  \frac{L^4}{\kappa^2} t^{1/9} \left( \sum_{s=1}^{t-1}f_n(s) \right)^2
\end{align*}

If we pick $t>\Omega\left( d! \kappa^2 C_3^2 / L^4 \right)^9$, we are able to get
\begin{align}
    & \left( \sum_{s=1}^{t-1}f_m(s)^2 \right) \left( \sum_{s=1}^{t-1}f_n(s)^2 \right) \geq  8 d! C_3^2 \left( \kappa t / 2 + \sum_{s=1}^{t-1}f_n(s) \right)^2 \\
\end{align}
\ug{TODO, cleanup.  \ref{ineq:diagonal} is not necessary.}
 which are combined with inequality~\ref{ineq:diagonal} to show for any $m\not = n$
 \begin{align*}
     & \left( \sum_{s=1}^{t-1}f_m(s)^2 \right) \left( \sum_{s=1}^{t-1}f_n(s)^2 \right) \geq  2 d! C_3^2 \left( \kappa t + \sum_{s=1}^{t-1}f_n(s)  + \sum_{s=1}^{t-1}f_n(s) \right)^2       
 \end{align*}
which is simply the following
 \begin{align*}
 \left| G_{n,m} \right| = \left| G_{m,n} \right| \leq \frac{1}{\sqrt{2d!}}\sqrt{G_{m,m} G_{n,n}}\\
 \end{align*}

\end{proof}

\begin{lemma}
Under the same condition of Lemma~\ref{lemma:digonal-dominance}, we have $\det(G) \geq \frac{1}{2}\prod_{i=1}^d G_{i,i}$
\end{lemma}

\begin{proof}
Now we show $\det(G)$ is dominated by its diagonal terms given Lemma~\ref{lemma:digonal-dominance}. In fact, by the Leibniz formula of determinant,
\begin{align*}
    \det(G)= \sum_{\sigma} \sign(\sigma)\prod_{i=1}^d G_{i, \sigma(i)} = \prod_{i=1}^d G_{i,i} + \sum_{\sigma\not= I} \sign(\sigma)\prod_{i=1}^d G_{i, \sigma(i)}
\end{align*}
Note that the second term's magnitude can be bounded in the following way.
\begin{align*}
    \left| \sum_{\sigma\not= I} \sign(\sigma)\prod_{i=1}^d G_{i, \sigma(i)} \right| & \leq \sum_{\sigma\not= I}  \left| \prod_{i=1}^d G_{i, \sigma(i)} \right|
    \leq  \sum_{\sigma\not= I}  \left| \prod_{i:i=\sigma(i)}^d G_{i, i} \right| \left| \prod_{i\not=\sigma(i)}G_{i, \sigma(i)} \right| \\
    & \leq   \sum_{\sigma\not= I}   \prod_{i:i=\sigma(i)}^d \left| G_{i, i} \right| \prod_{i\not=\sigma(i)} \left| G_{i, \sigma(i)} \right| \\
    & \leq   \sum_{\sigma\not= I}   \prod_{i:i=\sigma(i)}^d \left| G_{i, i} \right| \prod_{i\not=\sigma(i)} \frac{1}{\sqrt{2d!}} \sqrt{ G_{i,i}~
G_{\sigma(i), \sigma(i)} } \\
    & \leq   \sum_{\sigma\not= I}   \prod_{i:i=\sigma(i)}^d \left| G_{i, i} \right| \left( \frac{1}{\sqrt{2d!}} \right)^2 \prod_{i\not=\sigma(i)} G_{i,i} \\
    & \leq \frac{1}{2d!} \sum_{\sigma\not=I}\prod_{i=1}^d G_{i,i} \leq \frac{1}{2}\prod_{i=1}^d G_{i,i}
\end{align*}
where we use the fact that the indices set $\{i|i\not=\sigma(i)\}$ consists of cycles, which makes each $G_{i,i}$ appear exactly twice in the product $\prod_{i\not=\sigma(i)} \sqrt{ G_{i,i}~
G_{\sigma(i), \sigma(i)} }$.

Therefore, we obtain $\det(G)\geq (1-1/2) \prod_{i=1}^d G_{i,i} = \frac{1}{2}\prod_{i=1}^d G_{i,i} $.
\end{proof}

\begin{lemma}
Under the same condition of Lemma~\ref{lemma:digonal-dominance}, we have
\begin{align*}
G^{-1}\beta = O(t^{-2/9}) \begin{bmatrix}
f_1(t)^{-3/2}\\
f_2(t)^{-3/2} \\
\vdots\\
f_d(t)^{-3/2} \\
\end{bmatrix}
\end{align*}
\end{lemma}

\begin{proof}
By Cramer's rule,
\begin{align*}
    \left(G^{-1}\beta\right)_i = \det\left(\begin{bmatrix}
    G_{1,1} & \cdots & G_{1,i-1} & f_1(t) & G_{1, i+1} & \cdots& G_{1,d}\\
    \vdots  &         & \vdots  & \vdots  & \vdots     &       &    \vdots \\
    G_{i,1} & \cdots & G_{i,i-1} & f_i(t) & G_{i,i+1} & \cdots &G_{i,d}\\
    \vdots  &         & \vdots  & \vdots  & \vdots     &       &    \vdots \\
    G_{d,1} & \cdots & G_{d,i-1} & f_d(t) & G_{d, i+1} & \cdots& G_{d,d}\\
    \end{bmatrix}\right) / \det(G) \\
    \leq 2 \det\left(\begin{bmatrix}
    G_{1,1} & \cdots & G_{1,i-1} & f_1(t) & G_{1, i+1} & \cdots& G_{1,d}\\
    \vdots  &         & \vdots  & \vdots  & \vdots     &       &    \vdots \\
    G_{i,1} & \cdots & G_{i,i-1} & f_i(t) & G_{i,i+1} & \cdots &G_{i,d}\\
    \vdots  &         & \vdots  & \vdots  & \vdots     &       &    \vdots \\
    G_{d,1} & \cdots & G_{d,i-1} & f_d(t) & G_{d, i+1} & \cdots & G_{d,d}\\
    \end{bmatrix}\right) / \prod_{i=1}^d G_{i,i} \\
    \leq 2\det\left(\begin{bmatrix}
    1 & \cdots & \frac{f_1(t)}{\sqrt{G_{1,1}G_{i,i}}} & \cdots & \frac{G_{1,d}}{\sqrt{G_{1,1}G_{d,d}}}\\
    \vdots    &          & \vdots     &      &    \vdots \\
    \frac{G_{i,1}}{\sqrt{G_{1,1}, G_{i,i}}} & \cdots & \frac{f_i(t)}{G_{i,i}}  & \cdots & \frac{G_{i,d}}{\sqrt{G_{i,i}G_{d,d}}}\\
    \vdots  &         & \vdots  &   & \vdots    \\
    \frac{G_{d,1}}{\sqrt{G_{1,1}G_{d,d}}} & \cdots & \frac{f_d(t)}{\sqrt{G_{i,i}G_{d,d}}} & \cdots & 1 \\
    \end{bmatrix} \right)
\end{align*}

Using the conclusion of Lemma~\ref{lemma:digonal-dominance}, we know the off-diaognal entries' magnitude except for the $i$-th column  of the above matrix is at most $1 / \sqrt{2d!}$. Thus it follows that
\begin{align*}
    \left(G^{-1}\beta\right)_i &\leq 2 \left( \frac{f_i(t)}{G_{i,i}} + d! \left( \frac{1}{\sqrt{2d!}}\right)^2 \max_j \frac{f_j(t)}{\sqrt{G_{i,i}G_{j,j}}} \ \right)\\
    & \leq 2 \left( \frac{f_i(t)}{G_{i,i}} + \frac{1}{2\sqrt{G_{i,i}}} \max_j \frac{f_j(t)}{\sqrt{\sum_{s=1}^{t-1}f_j(s)^2}} \ \right) \\
    & \leq 2 \left( \frac{f_i(t)}{G_{i,i}} + \frac{C'}{2\sqrt{G_{i,i}}} \max_j \frac{f_j(t)}{\sqrt{(f_j(t) + L)^3 / L}} \ \right) \\
    & \leq 2 \left( \frac{f_i(t)}{G_{i,i}} + \frac{C' \sqrt{L}}{2\sqrt{G_{i,i}}} \max_j f_j(t)^{-1/2}  \right) \\
    & \leq 2 \left( \frac{f_i(t)}{G_{i,i}} + \frac{C'}{2\sqrt{G_{i,i}} \sqrt{t}} \right) \leq \frac{4C'}{\sqrt{tG_{i,i}}} \\
    & \leq C_5 f_i(t)^{-3/2} t^{-2/9}
\end{align*}

for some absolute constants $C'$ and $C_5$ where we use the assumption that $f_t(t) \geq L t^{4/9}$.

\end{proof}

\ug{Reordering the remaining probably makes sense if the following is of use.}

\begin{lemma}\label{lemma:small_noise}
Suppose  $G_{m,m} = \sum_{s=1}^{t-1}f_m(s)^2 \leq \gamma t$, then
$\sum_{s=1}^t \left| \left(V^{-1} \epsilon_s \right)_m  \right| \leq 4\kappa \gamma^{1/3}t$.
\end{lemma}
\begin{proof}
We first note that $f_m(s) \geq \gamma^{1/3}$ for at most $\gamma^{1/3}t$ time steps $s$.  \\

Now, suppose $f_m(s) \leq \gamma^{1/3}$.  If $ \left| \left(V^{-1} \epsilon_s \right)_m  \right| > 2\gamma^{1/3}$, then by the triangle inequality, $f_m(s+1) > \gamma^{1/3}$.  It follows that the only times where $ \left| \left(V^{-1} \epsilon_s \right)_m  \right| > 2\gamma^{1/3}$ occur when $f_m(s) \geq \gamma^{1/3}$ or $f_m(s+1) \geq \gamma^{1/3}$.  Noting that $ \left| \left(V^{-1} \epsilon_s \right)_m  \right| \leq \kappa$, we have

\begin{align*}
    \sum_{s=1}^t \left| \left(V^{-1} \epsilon_s \right)_m  \right| \leq 2\kappa \gamma^{1/3}t  + 2\gamma^{1/3}t \leq 4\kappa \gamma^{1/3}t 
\end{align*}

\end{proof}

\begin{lemma}
let $\gamma < 1$ and suppose $ G_{m,m}  \leq \gamma t$. Then we must have $\left| G_{n,m} \right| \leq O(t\gamma^{1/3}) $
\end{lemma}

\begin{proof}
Recalling \eqref{ineq:crossterm_bound}, we have 
\begin{align*}
    \left| G_{m,n} \right| & \leq C_3 \sum_{i=1}^{t-1}  \left| \left(V^{-1} x_i \right)_m  \left(\overline{V^{-1} \epsilon_i} \right)_n \right| 
    + \left| \left(V^{-1} \epsilon_i \right)_m \left(\overline{V^{-1} x_i} \right)_n \right| 
    + \left| \left(V^{-1} \epsilon_i \right)_m  \left(\overline{V^{-1} \epsilon_i}\right)_n \right| \\
    &\leq C_3 \left(\left( \sum_{i=1}^{t-1}  f_m(i)\right) 
    + \max_i \left|\left(\overline{V^{-1} x_i} \right)_n \right| \left(\sum_{i=1}^{t-1} \left| \left(V^{-1} \epsilon_i \right)_m \right|\right)
    + \sum_{i=1}^{t-1}\left| \left(V^{-1} \epsilon_i \right)_m \right|^2\right)
\end{align*}

First, we note that $\sum_{i=1}^{t-1}  f_m(i) \leq t\sqrt{\gamma}$ because $\sum_{s=1}^{t-1}f_m(s)^2 \leq \gamma t$ using $\|a\|_1 \leq \sqrt{t} \|a\|_2$.  The second term is then bounded by lemma~\ref{lemma:small_noise}.  The third term also uses this lemma and the fact that $\left| \left(V^{-1} \epsilon_i \right)_m \right|^2 \leq \kappa \left| \left(V^{-1} \epsilon_i \right)_m \right|$.
\end{proof}

\section{Conclusion}
\label{sec:conclusion}

Problems left open: Jordan blocks, lower bounds.

\section{Adversarial case: Main theorem and proof}

\begin{thm}
For the LDS problem, online Newton Step as described below attains regret
\begin{align*}
R_T&=O(C^2\ln (T(C_x+C_{A^*})))
\end{align*}
where
\begin{itemize}
\item
$\ve{A^*}\le R$.
\item
$\ve{x_1}\le C_x$.
\item
$\ve{V}_2\ve{V^{-1}}_2\le C_{A^*}$, where $A^*=V\La V^{-1}$ with $\La$ diagonal.
\item
The minimal polynomial $\sumz id a_i\la^i$ of $p$ satisfies $\sumz id |a_i|\le C_p$, where $a_d=0$.
\item
$C=R(C_x+C_{A^*}(C_p+d)d)$.
\end{itemize}•
\end{thm}

\begin{algorithm}[h!]
\begin{algorithmic}
\State Input: Description of convex sets $K_0\supeq K_1\supeq \cdots$, $x_1\in K_0\subeq \R^n$, parameters $\ga, \mu>0$.
\State Let $\Si_0=\mu I_n$.
\For{$t=1$ to $T$}
	\State Play $x_t$ and observe cost $f_t(x_t)$.
	\State Update $\Si_t = \Si_{t-1}+\nb_t \nb_t^\top$, where $\nb_t = \nb f_t(x_t)$.
	\State Update $x_{t+1} = \pi_{K_t}^{A_t}\pa{x_t - \rc{\ga}\Si_t^{-1}\nb_t}$, where $\pi_{K_t}^{\Si_t}$ denotes projection to $K_t$ in the norm $\ve{x}_{\Si_t} = x^\top \Si_t x$.
\EndFor
\end{algorithmic}
 \caption{Online Newton Step}
 \label{a:ons}
\end{algorithm}
We will use this algorithm with $A_1=0$ and 
\begin{align}
f_t(A) &= \ve{Ax_t-x_{t+1}}^2\\
K_t &= \set{A}{\ve{A}_F\le R \text{ and }
\forall s\le t,
\ve{Ax_s-x_{s+1}}_2\le 1
}.
\end{align}
%[NO] Note: For a quadratic objective, online Newton step with $\ga = 1$ is equivalent to online ridge regression.

\begin{df}
A twice-differentiable $f:\R^n\to \R$ is $\al$-exp-concave at $x$ iff $\nb^2 f(x) \succeq \al \nb f(x) \nb f(x)^\top$.
\end{df}

\begin{thm}
Algorithm~\ref{a:ons} with parameters
$\ga \le \al$,  %$\ga = \rc 2 \min\{\rc{4GD},\al\}$, 
$\mu = \rc{\ga^2D^2}$ and $T>4$ guarantees
\begin{align*}
R_T &\le %5\pa{\rc \al + GD}n \ln T.
\rc{2\ga} \pa{n\ln (TG^2D^2\ga+1)}.
\end{align*}
Here, $\al$ is such that each $f_t$ is $\al$-exp-concave at $x_t$, $\ve{\nb_t}\le G$, the diameter of $K_0$ is at most $D$. 
\end{thm}
\begin{proof}
See Theorem 4.3 in [OCO, Hazan]. The only changes are that we keep $\ga\le \al$ and  that we are projecting to a shrinking sequence of sets, $K_{t}$ at step $t$, instead of a fixed $K_0$. 
\fixme{I think the proof goes through! Check this carefully.}
\end{proof}

Note that $f(a) = \ve{a^\top x-b}^2$ is $\rc{2(a^\top x-b)^2}$-exp-concave at $a$, because 
\begin{align*}
\nb_a^2 f(a) &= 2xx^\top\\
\nb_a f(a) &= 2(a^\top x-b) x.
\end{align*}
From this, we get that $f(A) = \ve{A^\top x-b}^2$ is 
$\rc{\sumo jd 2(a_j^\top x-b_j)^2} = \rc{\ve{Ax-b}_2^2}$-exp-concave at $A$.

Suppose $A^*=V\La V^{-1}$ with $\ve{V}_2\ve{V^{-1}}_2\le C_{A^*}$ and $\La$ diagonal. Then $\ve{A^{*j}}\le C_{A^*}$ for all $j$. Let $p(\la) = \sumz id a_d\la^d$ be the minimal polynomial of $A^*$, where $a_d=1$. Suppose $\sumz id |a_d|\le C_p$.

For a sequence $x_t$, let $T$ be the operator defined by $(Tx)_t=x_{t-1}$.  Let $x'$ be the sequence defined by $x_s' = A^{*[s-(t-d)]}x_{t-d}$. Then $[p(T)x']_t=0$, and 
\begin{align}
p(T) x &= p(T)x' +\sumz id a_i \pa{\sumz j{d-1-i}A^{*j}\xi_{t-i-j}}\\
\ab{x_t  - \pa{\sumo i{d-1} -a_i x_{t-d+i}}}
&\le C_{A^*}C_pd.
\end{align}
Use the notation $\te(L)$ to denote a number of absolute value $\le L$.
Thus, if $t\ge d+1$, and $A\in K_{t-1}$, then 
\begin{align}
Ax_t &=-\sumz i{d-1} a_i Ax_{t-d+i} + \te(RC_{A^*} C_pd)\\
x_{t+1} &= -\sumz i{d-1} a_i x_{t-d+1+i} + \te(C_{A^*}C_p d)
\end{align}
so 
\begin{align*}
\ve{Ax_t - x_{t+1}}
&\le \sumz i{d-1} a_i \ve{Ax_{t-d+i} - x_{t-d+1+i}} + (R+1) C_{A^*} C_p d\\
&\le C_p + (R+1) C_{A^*} C_p d
\le O(RC_{A^*}C_pd).
\end{align*}
We also bound the discrepancy for $t\le d$. Suppose $\ve{x_1}\le C_x$. For $t\le d$,
\begin{align*}
\ve{x_t} &\le \ve{x_1} + (t-1)^2C_{A^*} \le C_x + t^2 C_{A^*}.
\end{align*}
%Supposing $d\le C_p$, we get
We get
\begin{align*}
\ve{Ax_t-x_{t+1}} &\le R(C_x + d^2 C_{A^*}) %= RC_x + RC_{A^*}C_pd.
\end{align*}
Thus we have, at each step $t$, that 
\begin{align*}
\ve{A_tx_t-x_{t+1}}&\le O(RC_x + RC_{A^*}(C_p+d)d).
\end{align*}
Let $C=RC_x + RC_{A^*}(C_p+d)d$.
This means that 
\begin{itemize}
\item
Because $\nb_A[ \ve{A x_t-x_{t+1}}^2] = (Ax_t-x_{t+1})x_t^\top$, the maximum gradient is bounded by $G=O(C(C_x + T^2 C_{A^*}))$.
\item
We can take $\rc{\al}=\Te(C^2)$.
\item
The diameter is $2R$.
\end{itemize}
Thus taking $\ga=\al$ we obtain a regret bound of
\begin{align*}
R_T &=O\pa{\rc{\al} \ln (TG^2D^2\al + 1)}\\
&= O\pa{C^2\ln \pa{TC^2(C_x+T^2C_{A^*})^2/C^2 + 1}}\\
&= O\pa{C^2 \ln (T(C_x+C_{A^*}))}.
\end{align*}

==> ons.tex <==
\section{Adversarial case: Main theorem and proof}

\begin{thm}
For the LDS problem, online Newton Step as described below attains regret
\begin{align*}
R_T&=O(C^2\ln (T(C_x+C_{A^*})))
\end{align*}
where
\begin{itemize}
\item
$\ve{A^*}\le R$.
\item
$\ve{x_1}\le C_x$.
\item
$\ve{V}_2\ve{V^{-1}}_2\le C_{A^*}$, where $A^*=V\La V^{-1}$ with $\La$ diagonal.
\item
The minimal polynomial $\sumz id a_i\la^i$ of $p$ satisfies $\sumz id |a_i|\le C_p$, where $a_d=0$.
\item
$C=R(C_x+C_{A^*}(C_p+d)d)$.
\end{itemize}•
\end{thm}

\begin{algorithm}[h!]
\begin{algorithmic}
\State Input: Description of convex sets $K_0\supeq K_1\supeq \cdots$, $x_1\in K_0\subeq \R^n$, parameters $\ga, \mu>0$.
\State Let $\Si_0=\mu I_n$.
\For{$t=1$ to $T$}
	\State Play $x_t$ and observe cost $f_t(x_t)$.
	\State Update $\Si_t = \Si_{t-1}+\nb_t \nb_t^\top$, where $\nb_t = \nb f_t(x_t)$.
	\State Update $x_{t+1} = \pi_{K_t}^{A_t}\pa{x_t - \rc{\ga}\Si_t^{-1}\nb_t}$, where $\pi_{K_t}^{\Si_t}$ denotes projection to $K_t$ in the norm $\ve{x}_{\Si_t} = x^\top \Si_t x$.
\EndFor
\end{algorithmic}
 \caption{Online Newton Step}
 \label{a:ons}
\end{algorithm}
We will use this algorithm with $A_1=0$ and 
\begin{align}
f_t(A) &= \ve{Ax_t-x_{t+1}}^2\\
K_t &= \set{A}{\ve{A}_F\le R \text{ and }
\forall s\le t,
\ve{Ax_s-x_{s+1}}_2\le 1
}.
\end{align}
%[NO] Note: For a quadratic objective, online Newton step with $\ga = 1$ is equivalent to online ridge regression.

\begin{df}
A twice-differentiable $f:\R^n\to \R$ is $\al$-exp-concave at $x$ iff $\nb^2 f(x) \succeq \al \nb f(x) \nb f(x)^\top$.
\end{df}

\begin{thm}
Algorithm~\ref{a:ons} with parameters
$\ga \le \al$,  %$\ga = \rc 2 \min\{\rc{4GD},\al\}$, 
$\mu = \rc{\ga^2D^2}$ and $T>4$ guarantees
\begin{align*}
R_T &\le %5\pa{\rc \al + GD}n \ln T.
\rc{2\ga} \pa{n\ln (TG^2D^2\ga+1)}.
\end{align*}
Here, $\al$ is such that each $f_t$ is $\al$-exp-concave at $x_t$, $\ve{\nb_t}\le G$, the diameter of $K_0$ is at most $D$. 
\end{thm}
\begin{proof}
See Theorem 4.3 in [OCO, Hazan]. The only changes are that we keep $\ga\le \al$ and  that we are projecting to a shrinking sequence of sets, $K_{t}$ at step $t$, instead of a fixed $K_0$. 
\fixme{I think the proof goes through! Check this carefully.}
\end{proof}

Note that $f(a) = \ve{a^\top x-b}^2$ is $\rc{2(a^\top x-b)^2}$-exp-concave at $a$, because 
\begin{align*}
\nb_a^2 f(a) &= 2xx^\top\\
\nb_a f(a) &= 2(a^\top x-b) x.
\end{align*}
From this, we get that $f(A) = \ve{A^\top x-b}^2$ is 
$\rc{\sumo jd 2(a_j^\top x-b_j)^2} = \rc{\ve{Ax-b}_2^2}$-exp-concave at $A$.

Suppose $A^*=V\La V^{-1}$ with $\ve{V}_2\ve{V^{-1}}_2\le C_{A^*}$ and $\La$ diagonal. Then $\ve{A^{*j}}\le C_{A^*}$ for all $j$. Let $p(\la) = \sumz id a_d\la^d$ be the minimal polynomial of $A^*$, where $a_d=1$. Suppose $\sumz id |a_d|\le C_p$.

For a sequence $x_t$, let $T$ be the operator defined by $(Tx)_t=x_{t-1}$.  Let $x'$ be the sequence defined by $x_s' = A^{*[s-(t-d)]}x_{t-d}$. Then $[p(T)x']_t=0$, and 
\begin{align}
p(T) x &= p(T)x' +\sumz id a_i \pa{\sumz j{d-1-i}A^{*j}\xi_{t-i-j}}\\
\ab{x_t  - \pa{\sumo i{d-1} -a_i x_{t-d+i}}}
&\le C_{A^*}C_pd.
\end{align}
Use the notation $\te(L)$ to denote a number of absolute value $\le L$.
Thus, if $t\ge d+1$, and $A\in K_{t-1}$, then 
\begin{align}
Ax_t &=-\sumz i{d-1} a_i Ax_{t-d+i} + \te(RC_{A^*} C_pd)\\
x_{t+1} &= -\sumz i{d-1} a_i x_{t-d+1+i} + \te(C_{A^*}C_p d)
\end{align}
so 
\begin{align*}
\ve{Ax_t - x_{t+1}}
&\le \sumz i{d-1} a_i \ve{Ax_{t-d+i} - x_{t-d+1+i}} + (R+1) C_{A^*} C_p d\\
&\le C_p + (R+1) C_{A^*} C_p d
\le O(RC_{A^*}C_pd).
\end{align*}
We also bound the discrepancy for $t\le d$. Suppose $\ve{x_1}\le C_x$. For $t\le d$,
\begin{align*}
\ve{x_t} &\le \ve{x_1} + (t-1)^2C_{A^*} \le C_x + t^2 C_{A^*}.
\end{align*}
%Supposing $d\le C_p$, we get
We get
\begin{align*}
\ve{Ax_t-x_{t+1}} &\le R(C_x + d^2 C_{A^*}) %= RC_x + RC_{A^*}C_pd.
\end{align*}
Thus we have, at each step $t$, that 
\begin{align*}
\ve{A_tx_t-x_{t+1}}&\le O(RC_x + RC_{A^*}(C_p+d)d).
\end{align*}
Let $C=RC_x + RC_{A^*}(C_p+d)d$.
This means that 
\begin{itemize}
\item
Because $\nb_A[ \ve{A x_t-x_{t+1}}^2] = (Ax_t-x_{t+1})x_t^\top$, the maximum gradient is bounded by $G=O(C(C_x + T^2 C_{A^*}))$.
\item
We can take $\rc{\al}=\Te(C^2)$.
\item
The diameter is $2R$.
\end{itemize}
Thus taking $\ga=\al$ we obtain a regret bound of
\begin{align*}
R_T &=O\pa{\rc{\al} \ln (TG^2D^2\al + 1)}\\
&= O\pa{C^2\ln \pa{TC^2(C_x+T^2C_{A^*})^2/C^2 + 1}}\\
&= O\pa{C^2 \ln (T(C_x+C_{A^*}))}.
\end{align*}

==> proof23.tex <==
\section{Proof}
\begin{thm}[Online ridge regression]
Consider the online linear regression problem, where at step $t$, one plays a matrix $A_t\in \R^{m\times n}$ and suffers loss $\ve{A_tx_t-y_t}^2$. Suppose that $\ve{x_t}\le B$ for all $t$. Define the regret with respect to $A$ by 
\begin{align}
R_T(A) &=\sumo tT \ve{A_tx_t-y_t}_2^2 - %\min_A 
\sumo tT \ve{Ax_t-y_t}_2^2.
\end{align}
Then online ridge regression with regularization parameter $\mu$ incurs regret
\begin{align}
R_T (A)&\le 
\mu \ve{A}_F^2 + \max_{1\le t\le T}\ve{y_t-A_tx_t}_2^2mn
\ln \pa{1+\fc{TB^2}n}.
\end{align}
\end{thm}

\begin{proof}
See \url{https://people.eecs.berkeley.edu/~bartlett/courses/281b-sp08/24.pdf}.
\end{proof}

In our case, $y_t=x_{t+1}$, and 
\begin{align}
A_t &=\amin_A \ba{\mu \ve{A}_F^2 + \sumo s{t-1} \ve{x_{s+1} - A x_s}_2^2}\\
&= \sumo s{t-1} x_{s+1} x_s^\top \pa{\mu I + \sumo s{t-1} x_s x_s^\top}^{-1}\\
&= \sumo s{t-1} (A^*x_s+\xi_{s+1}) x_s^\top \pa{\mu I + \sumo s{t-1} x_s x_s^\top}^{-1}
\end{align}
Noting that
\begin{align}
A^*&=\sumo s{t-1} (A^*x_s) x_s^\top \pa{\mu I + \sumo s{t-1} x_s x_s^\top}^{-1}
+ \mu \pa{\mu I + \sumo s{t-1} x_s x_s^\top}^{-1}
\end{align}
we get from subtracting that
\begin{align}
A_t x_t -x_{t+1} &= A_t x_t - A^*x_t - \xi_{t+1}\\
&=
\sumo s{t-1} \xi_{s+1} x_s^\top \pa{\mu I + \sumo s{t-1} x_s x_s^\top}^{-1} -  \mu \pa{\mu I + \sumo s{t-1} x_s x_s^\top}^{-1}
- \xi_{t+1}.
\end{align}
We proceed by bounding the first term. First, consider the one-dimensional case under a general condition that the $x_t$'s do not grow too rapidly.

\begin{lem}
Let $c,c_1,c_2$ be constants, $c_1\le \rc 2$, $c\ge \rc{c_1}$. 
Suppose that $x_s$ is a sequence such that if $|x_t|\ge c$, then there exist at least $c_1m$ indices $s<t$ such that $|x_s|\ge c_2 m$. Suppose $|\xi_s|\le 1$ for each $s$. Then 
\begin{align*}
\ab{\sumo s{t-1} \xi_{s+1} x_s \pa{\mu + \sumo s{t-1} x_s^2}^{-1}x_t}\le 
O\pa{
\max\bc{
\fc{ct}{\mu}, \rc{c_2^2}, \fc{t^{\rc 2}}{c_1^{\rc 3} c_2^{\fc 23}\mu^{\rc 6}}
}
}.
\end{align*}
\end{lem}
The regret scales as the square of this quantity, plus a term scaling as $\mu$. To balance the terms, we set $\pf{t^{\rc 2}}{\mu^{\rc 6}}^2\sim \mu$, so $\mu = t^{\fc 34}$ with regret $\wt O(t^{\fc 34})$.
\begin{proof}
%We may assume all the $x_s$ are nonnegative, by replacing $x_s$ by $|x_s|$.
Let $m=\max_{1\le s\le t-1} |x_s|$. 

First suppose $m<c$. Then 
\begin{align}
\ab{\sumo s{t-1} \xi_{s+1} x_s \pa{\mu + \sumo s{t-1} x_s^2}^{-1}x_t}\le 
\fc{ct}{\mu}.
\end{align}

%For the remainder of the proof, 
Now suppose $m\ge c$.
%problem with J blocks
Then there exists a subsequence $x_{i_1},\ldots, x_{i_n}$ where $n = \ce{c_1m}$ and $|x_{i_j}|\ge c_2m$ and $|x_{i_n}|=m$. Let $S=\{i_1,\ldots, i_n\}$. We have
\begin{align}
\sumo kn |x_{i_k}| &\le \ce{c_1 m}c=O(c_1m^2)&
\sumo kn x_{i_k}^2 &\ge \ce{c_1 m} (c_2m)^2 = \Omega(c_1c_2^2m^3)
\end{align}
Thus
\begin{align}
\fc{{{\sumo s{t-1} |x_s|}}}{\mu+\sumo s{t-1}x_s^2}
&\precsim
\fc{c_1 m^2+\sum_{i\in [t-1]\bs S} |x_{i}|}{\mu+c_1c_2^2 m^3+ \sum_{i\in [t-1]\bs S} x_{i}^2}\\
&\le
\max_{0\le x'_i\le m\text{ for }1\le i\le t-1-m} 
\fc{c_1 m^2+\sumo i{t-1-n} x_i'}{\mu+c_1c_2^2 m^3+\sumo i{t-1-n} x_i^{\prime2}}\\
&\le \max_{0\le x\le m}
\fc{c_1 m^2+(t-1-n) x}{\mu+c_1c_2^2 m^3+(t-1-n) x^2}
\end{align}
where the last inequality follows by Jensen's inequality since $x\mapsto x^2$ is convex (holding $\sumo i{t-1-n} x_i'$ constant, the smallest value of $\sumo i{t-1-n}x_i^{\prime 2}$ is attained when they are equal). Continuing,
\begin{align}
&\le \max_{0\le x\le m} \pa{\fc{c_1m^2}{\mu + c_1c_2^2m^3} + \fc{(t-1-n)x}{\mu+c_1c_2^2 m^3+(t-1-n) x^2}
}\\
&\le \max_{0\le x\le m} \pa{\fc{c_1m^2}{\mu + c_1c_2^2m^3} + \fc{tx}{\mu+c_1c_2^2 m^3+t x^2}
}
\end{align}
because $x\mapsto \fc{ax}{b+cx}$ is increasing for $a,b,c>0$ and $x\ge 0$.
%The function $t\mapsto \fc{a+tb}{c+td} = \fc bd + \fc{a-\fc{bc}d}{c+td}$ is either increasing or decreasing, so this is at most $\max_{c\le x\le m} \bc{\fc{c_1m^2}{\mu + c_1c_2^2m^3}, \fc{c_1m^2 + tx}{\mu + c_1c_2^2m^3 + tx^2}}$. 
Thus
\begin{align}
\fc{{\pa{\sumo s{t-1} |x_s|}|x_t|}}{\mu+\sumo s{t-1}x_s^2}
&\precsim
m\cdot 
\max_{0\le x\le m} \pa{\fc{c_1m^2}{\mu + c_1c_2^2m^3} + \fc{tx}{\mu+c_1c_2^2 m^3+tx^2}
}\\
&\le 
\max_{0\le x\le m} \pa{\fc{1}{c_2^2} + \fc{mtx}{\mu+c_1c_2^2 m^3+t x^2}
}
\end{align}
The second term is bounded by
\begin{align}
\pf{mtx}{\mu}^{\fc 16}
\pf{mtx}{c_1c_2^2m^3}^{\fc 26}
\pf{mtx}{tx^2}^{\fc 36}
&\le \fc{ t^{\rc 2}}{c_1^{\fc 13}c_2^{\fc 23}\mu^{\fc 16}}.
\end{align}
%\fixme{First, if $t-1-n\le m$, then $(t-1-n) x=O(m^2)$ and $(t-1-n) x^2=O(m^3)$. So assume $t-1-n>m$, so that %$(t-1-n)x^2 = \Om(tx^2)$. 
%the above is $\precsim \fc{m^2 + tx}{m^3 + tx^2}$. }
%Consider 3 cases.
%\begin{enumerate}
%\item
%$tx\le c_1 m^2$: Then the numerator is dominated by $c_1 m^2$ so this is $\le m\cdot \fc{c_1 m^2}{c_1c_2^2 m^3}\le \rc{c_2^2}$.
%\item
%$tx>c_1 m^2$, $tx^2\ge c_1c_2^2 m^3$: Then the denominator is dominated by $tx^2$ so this is $\precsim m\cdot\fc{tx}{tx^2} = \fc{m}x$. From $tx^2\ge c_1c_2^2 m^3$, we get $\fc{m^3}{x^3}\le \fc t{xc_1c_2^2}...=O(t)$ (using $x\ge c$) so $\fc{m}x = O(t^{\rc 3})$.
%\item
%$tx>m^2$; $tx^2<m^3$: Then the denominator is dominated by $m^3$ so this is $\precsim \fc{tx}{m^3}=t \rc{m^2} \fc xm$. Now $m^3>t$ implies $m>t^{\rc 3}$ so $t\rc{m^2}\fc xm< t\rc{t^{\fc 23}}\le t^{\rc 3}$.
%\end{enumerate}
%Finally, the bound can be attained by $\ub{1,\ldots, 1}{t-\fl{t^{\rc 3}}}, 2, \ldots, \fl{t^{\rc 3}}$.
\end{proof}

==> random.tex <==
\section{Random case}

When the noise has no large Fourier coefficient, we don't have to suffer the $C_p$ factor (which may be as large as $2^d$).

\begin{enumerate}
    \item Known state (same setting as before)
    \item Autoregression  on previous inputs and outputs.
        \begin{enumerate}
            \item Kalman filter - hidden state. (cf. exponential forgetting in~\cite{Kozdoba2018OnLineLO}. Unlike them, if we assume Fourier-random input, we should be able to not suffer a factor of $\max \ve{h_t}$.) $L^1$ Fourier regression on inputs should be more sample-efficient than $L^2$ regression. This should make a noticeable difference when there is LOW process noise and HIGH observation noise.
        \end{enumerate}
\end{enumerate}
